Local-Global MCMC kernels: the best of both worlds

Recent works leveraging learning to enhance sampling have shown promising results, in particular by designing effective non-local moves and global proposals. However, learning accuracy is inevitably limited in regions where little data is available such as in the tails of distributions as well as in high-dimensional problems. In the present paper we study an Explore-Exploit Markov chain Monte Carlo strategy ($Ex^2MCMC$) that combines local and global samplers showing that it enjoys the advantages of both approaches. We prove $V$-uniform geometric ergodicity of $Ex^2MCMC$ without requiring a uniform adaptation of the global sampler to the target distribution. We also compute explicit bounds on the mixing rate of the Explore-Exploit strategy under realistic conditions. Moreover, we also analyze an adaptive version of the strategy ($FlEx^2MCMC$) where a normalizing flow is trained while sampling to serve as a proposal for global moves. We illustrate the efficiency of $Ex^2MCMC$ and its adaptive version on classical sampling benchmarks as well as in sampling high-dimensional distributions defined by Generative Adversarial Networks seen as Energy Based Models. We provide the code to reproduce the experiments at the link: https://github.com/svsamsonov/ex2mcmc_new.

==> Local - (learned) Global Mixed Kernels/algo_ex2.tex <==
\begin{algorithm2e}[t!]
    \SetKwInOut{In}{Input}
    \SetKwInOut{Out}{Output}
    \caption{Single stage of \XTryM\ algorithm with independent proposals}
    \label{alg:X-Try-MCMC}
    \SetKwFunction{KwPrint}{print}
    \SetKwProg{Fn}{Procedure \ }{:}{end}
    \SetKwFunction{X-Try}{X-Try SIR}
    \SetKwProg{myalg}{Algorithm}{}{}
    \Fn{\XTryM\ $(Y_k,\proposal,\rejukernel)$}{
    \In{Previous state $Y_{k}$; proposal distribution $\proposal$; rejuvenation kernel $\rejukernel$;}
    \Out{New sample $Y_{k+1}$; pool of proposals $\chunku{X}{2}{N}_{k+1} \sim \proposal$;}
    $Z_{k+1}\eqsp, \chunku{X}{2}{N}_{k+1} = \isir(Y_{k},\proposal)$; \\
    Draw $Y_{k+1} \sim \rejukernel(Z_{k+1},\cdot)$. \\
    %For $i \in \range{N}$, compute the normalized weights $\unormweight_i[k+1]= \weightfunc(X^{i}[k+1])$. \\
    %Compute $\NormFactor[k+1] = \sum_{i=1}^N \unormweight_i[k+1]$. \\
    %\For{$i \in \range{N}$}{
    %    compute the normalized weights $\normweight_{i,k+1}= \weightfunc(X^{i}_{k+1})/\sum_{\ell=1}^N\weightfunc(X^{\ell}_{k+1})$; \\
    %    }
    %Draw the proposal index $I_{k+1} \sim \mathrm{Cat}(\normweight_{1,k+1},\dots,\normweight_{N,k+1})$; \\
    %Draw  $Y_{k+1}\sim \rejukernel(X^{I_{k+1}}_{k+1},\cdot)$. \\
    }
    \vspace{-3pt}
\end{algorithm2e} 
\vspace{-3mm}

==> Local - (learned) Global Mixed Kernels/algo_flex.tex <==
 \begin{algorithm2e}[t!]
    \caption{Single stage of \FlXTryM. Steps of \XTryM\ use the NF proposal with parameters $\theta_k$. Step $4$ updates the parameters using the gradient estimate obtained from all the chains.}
    \label{alg:NF-X-Try-MCMC}
    \SetKwInOut{In}{Input}
    \SetKwInOut{Out}{Output}
    \SetKwFunction{KwPrint}{print}
    \SetKwProg{Fn}{Function}{:}{end}
    \SetKwFunction{X-Try}{X-Try SIR}
    \SetKwProg{myalg}{Algorithm}{}{}
    \In{weights $\theta_k$, batch $Y_{k}[1:M]$}
    \Out{new weights $\theta_{k+1}$, batch $Y_{k+1}[1:M]$}
    \For{$j \in \range{M}$}{
        $Y_{k+1}[j] %= \isir\ (Y_k[j],\pushforward[T_{\theta_k}][\Lambda])$
        = \XTryM\ (Y_k,\pushforward[T_{\theta_k}][\proposalbase],\rejukernel)$
    }
    Draw ${Z}[1:M] \sim \proposalbase$.\\
    % Update $\theta_{k+1} = \theta_{k} - \gamma \widehat{\nabla\mathcal{L}}(Y_{k+1}, \bar{Z}, \theta_k)$.
    Update $\theta_k= \theta_{k-1} + \gamma_k M^{-1} \sum_{j=1}^M  H(\theta_{k-1},\chunku{X_k}{1}{N}[j],\chunku{Z_k}{2}{N}[j])$ 
 \end{algorithm2e}

==> Local - (learned) Global Mixed Kernels/algo_isir.tex <==
\begin{algorithm2e}[t!]
    \SetKwInOut{In}{Input}
    \SetKwInOut{Out}{Output}
    \caption{Single stage of \isir\ algorithm with independent proposals}
    \label{alg:i-sir-MCMC}
    \SetKwFunction{KwPrint}{print}
    \SetKwProg{Fn}{Procedure \ }{:}{end}
    \SetKwFunction{X-Try}{iterated SIR}
    \SetKwProg{myalg}{Algorithm}{}{}
    \Fn{\isir\ $(Y_k,\proposal)$}{
    \In{Previous state $Y_{k}$; proposal distribution $\proposal$;}
    \Out{New state $Y_{k+1}$; pool of proposals $\chunku{X}{2}{N}_{k+1} \sim \proposal$;}
    Set $X^1_{k+1}= Y_{k}$, draw $\chunku{X}{2}{N}_{k+1} \sim \proposal$; 
    \For{$i \in \range{N}$}{
        compute the normalized weights $\normweight_{i,k+1}= \weightfunc(X^{i}_{k+1})/\sum_{\ell=1}^N\weightfunc(X^{\ell}_{k+1})$; \\
        }
    Draw the proposal index $I_{k+1} \sim \mathrm{Cat}(\normweight_{1,k+1},\dots,\normweight_{N,k+1})$; \\
    Set $Y_{k+1} := X^{I_{k+1}}_{k+1}$. \\
    }
\vspace{-3pt}
\end{algorithm2e} 


==> Local - (learned) Global Mixed Kernels/conclusion.tex <==
\vspace{-3mm}
%\marylou{Tuning down the allegation of novelty - the combination is relatively simple}
The present paper examines the benefits of combining local and global samplers. From a theoretical point of view, we show that global samplers are more robust when coupled with local samplers. Namely, a $V$-geometric ergodicity is obtained for the $\XTryM$ kernel under minimal assumptions. Meanwhile, the global samplers drives exploration when properly adjusted. Therefore, we also describe the adaptive version $\FlXTryM$ of the strategy involving the learning of a global proposal parametrized by a normalizing flow. We also check for the learning convergence along the adaptive MCMC run. Finally, a series of numerical experiments confirms the superiority of the strategy, including the high-dimensional examples.
While the startegy was described and analyzed for the \isir~global kernel, we note that it would be possible to extend the theory to other independent global samplers. We expect that the benefit of the combination would remain. Further studies of \FlXTryM, in particular the derivation of its mixing rate, is an interesting direction for future work.
% We propose a new MCMC algorithm, \XTryM, which allows to improve over the competitors due to the efficiency both at exploration and exploitation steps. We analyze its theoretical properties and suggest an adaptive version of the algorithm, \FlXTryM, based on normalizing flows. It allows to overcome the issues of MTM and \isir\ algorithms, which are caused by low acceptance rate when sampling from high dimensional distributions. Further studies of \FlXTryM, in particular its mixing rate, is an interesting direction for the future work

==> Local - (learned) Global Mixed Kernels/def.tex <==

\newcommand{\changes}[1]{{\color{violet}#1}}

\def\taumix{t_{\operatorname{mix}}}
\newcommand{\dobrush}{\mathsf{\Delta}}
\newcommandx{\dobru}[3][1=,3=]{\dobrush_{#1}^{#3}( #2)}

%%% aathsf
\def\msi{\mathsf{I}}
\def\msa{\mathsf{A}}
\def\tmsa{\tilde{\msa}}
\def\msd{\mathsf{D}}
\def\msz{\mathsf{Z}}
\def\msk{\mathsf{K}}
\def\mss{\mathsf{S}}
\def\msn{\mathsf{N}}
\def\msat{\tilde{\mathsf{A}}}
\def\msb{\mathsf{B}}
\def\msc{\mathsf{C}}
\def\mse{\mathsf{E}}
\def\msf{\mathsf{F}}
\def\mso{\mathsf{o}}
\def\msg{\mathsf{G}}
\def\msh{\mathsf{H}}
\def\msm{\mathsf{M}}
\def\msu{\mathsf{U}}
\def\msv{\mathsf{V}}
\def\msr{\mathsf{R}}
\newcommand{\msff}[2]{\mathsf{F}_{#1}^{#2}}
\def\msp{\mathsf{P}}
\def\msq{\mathsf{Q}}
\def\msx{\mathsf{X}}
\def\msy{\mathsf{Y}}



%%
\newcommandx{\CPE}[3][1=]{{\mathbb E}_{#1}\left[\left. #2 \, \right| #3 \right]} %%%% esperance conditionnelle
\newcommandx{\CPP}[3][1=]{{\mathbb P}_{#1}\left[\left. #2 \, \right| #3 \right]} %%%% esperance conditionnelle

%% mathcal
\def\NC{\mathcal{N}}
\def\mca{\mathcal{A}}
\def\mcz{\mathcal{Z}}
\def\mcat{\tilde{\mathcal{A}}}
\def\mcab{\bar{\mathcal{A}}}
\def\mcbb{\mathcal{B}}  %%% \mcb est déjà pris
\newcommand{\mcb}[1]{\mathcal{B}(#1)}
\def\mcc{\mathcal{C}}
\def\mcy{\mathcal{Y}}
\def\mcx{\mathcal{X}}
\def\mce{\mathcal{E}}
\def\mcf{\mathcal{F}}
\def\mcg{\mathcal{G}}
\def\mch{\mathcal{H}}
\def\mcm{\mathcal{M}}
\def\mcu{\mathcal{U}}
\def\mcv{\mathcal{V}}
\def\mcr{\mathcal{R}}
\newcommand{\mcff}[2]{\mathcal{F}_{#1}^{#2}}
\def\mcfb{\bar{\mathcal{F}}}
\def\bmcf{\bar{\mathcal{F}}}
\def\mcft{\tilde{\mathcal{F}}}
\def\tmcf{\tilde{\mathcal{F}}}
\def\mcp{\mathcal{P}}
\def\mcq{\mathcal{Q}}
\def\mct{\mathcal{T}}

%% mathbb
\def\rset{\mathbb{R}}
\def\rsets{\mathbb{R}^*}
\def\cset{\mathbb{C}}
\def\zset{\mathbb{Z}}
\def\nset{\mathbb{N}}
\def\nsets{\mathbb{N}^*}
\def\qset{\mathbb{Q}}
\def\Rset{\mathbb{R}}
\def\Cset{\mathbb{C}}
\def\Zset{\mathbb{Z}}
\def\Nset{\mathbb{N}}
\def\Tset{\mathbb{T}}

%%%% mathrm
\def\rmb{\mathrm{b}}
\def\mrb{\mathrm{b}}
\def\rmd{\mathrm{d}}
\def\rmZ{\mathrm{Z}}
\def\mrd{\mathrm{d}}
\def\mre{\mathrm{e}}
\def\rme{\mathrm{e}}
\def\rmn{\mathrm{n}}
\def\mrn{\mathrm{n}}
\def\mrc{\mathrm{C}}
\def\mrcc{\mathrm{c}}
\def\rmc{\mathrm{C}}
\def\rmC{\mathrm{C}}
\def\rmcc{\mathrm{c}}
\def\rma{\mathrm{a}}
\def\mra{\mathrm{a}}
\def\rmF{\mathrm{F}}
\def\rmE{\mathrm{E}}



\def\Tr{\operatorname{T}}
\def\trace{\operatorname{Tr}}
\newcommandx{\functionspace}[2][1=+]{\mathbb{F}_{#1}(#2)}
%% argmin, argmax
\newcommand{\argmax}{\operatorname*{arg\,max}}
\newcommand{\argmin}{\operatorname*{arg\,min}}
\newcommand{\1}{\mathbbm{1}}


\newcommand{\LeftEqNo}{\let\veqno\@@leqno}


\newcommand{\PE}{\mathbb{E}}
\def\PVar{\operatorname{Var}}
\newcommandx{\bconst}[1][1=]{\ensuremath{\mathsf{b}_{#1}}}
\newcommandx{\cconst}[1][1=]{\ensuremath{c_{#1}}}
\newcommandx{\rate}[1][1=]{\ensuremath{\tilde{\kappa}_{#1}}}
\newcommandx{\dconst}[1][1=]{\ensuremath{d_{#1}}}
\def\Csetfunction{\mathrm{C}}
\def\Kmala{\operatorname{K}}
\def\Rmalag{R_\step}
\def\Rmala{R}
\def\rmala{r}
\def\rula{r}
\def\alphamalan{\tau_{\step_n}^{\scriptscriptstyle{\operatorname{MALA}}}}
\def\Ltt{\mathtt{L}}
\def\Lttbeta{\mathtt{L}_{\beta}}
\def\Mtt{\mathtt{M}}
\def\Ctt{\mathtt{C}}
\def\rmD{\mathrm{D}}
\def\mrD{\mathrm{D}}
\def\mtt{\mathtt{m}}
\def\Ktt{\mathtt{K}}
\def\tKtt{\tilde{\mathtt{K}}}


\newcommandx{\pushforward}[2][1=T,2=\Lambda]{ {#1} \# {#2}}
\newcommandx{\VnormEq}[2][1=V]{\left\| #2 \right\|_{#1}}
\newcommandx{\norm}[2][1=]{\ifthenelse{\equal{#1}{}}{\Vert #2 \Vert}{\Vert #2 \Vert^{#1}}}


\def\bareta{\bar{\eta}}
\def\bgamma{\bar{\step}}
\def\tildem{\varpi}
\def\barb{\bar{b}}
\def\MKula{\mathrm{Q}^{\text{ULA}}}
\def\step{\gamma}
\newcommand{\normdens}{\boldsymbol{\varphi}}
\newcommand{\parentheseDeux}[1]{\left[ #1 \right]}
\def\alphaMALA{\alpha_{\gamma}}
\def\Rrm{M}


\newcommand{\PP}{\mathbb{P}}
% Operands
\newcommand{\tvnorm}[1]{\| #1 \|_{\mathrm{TV}}}
\newcommandx{\Vnorm}[2][1=V]{\| #2 \|_{#1}}

\newcommand{\ps}[2]{\left\langle#1,#2 \right\rangle}

\newcommand{\eqdef}{{:=}}

% Relations

\def\ie{\textit{i.e.}}
\def\eqsp{\;}
\newcommand{\coint}[1]{\left[#1\right)}
\newcommand{\ocint}[1]{\left(#1\right]}
\newcommand{\ooint}[1]{\left(#1\right)}
\newcommand{\ccint}[1]{\left[#1\right]}
\newcommand{\cointLigne}[1]{[#1)}
\newcommand{\ocintLigne}[1]{(#1]}
\newcommand{\oointLigne}[1]{(#1)}
\newcommand{\ccintLigne}[1]{[#1]}






\newcommand{\indi}[1]{\1_{#1}}
\newcommand{\indiacc}[1]{\1_{\{ #1 \}}}
\newcommand{\indiaccl}[1]{\1\left\{ #1 \right\}}
\newcommand{\ball}[2]{\operatorname{B}(#1,#2)}
\newcommand{\diameter}{\operatorname{diam}}
\def\Cat{\operatorname{Cat}}



\newcommand{\alain}[1]{\todo[color=blue!20]{{\bf AD:} #1}}
\newcommand{\eric}[1]{\todo[color=black!20]{{\bf EM:} #1}}
\newcommand{\som}[1]{\todo[color=red!20]{{\bf SS:} #1}}
\newcommand{\maxk}[1]{\todo[color=green!20]{{\bf MK:} #1}}
\newcommand{\marylou}[1]{\todo[color=orange!20]{{\bf MG:} #1}}

 \newcommand{\tcr}[1]{\textcolor{red}{#1}}
% \newcommand{\tcb}[1]{\textcolor{blue}{#1}}


\def\as{\ensuremath{\text{a.s.}}}
\def\dist{\operatorname{dist}}


\newcommandx\sequenceg[3][2=,3=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{( #1_{#2})}}{\ensuremath{( #1_{#2})_{ #2 \geq #3}}}}

\newcommandx\sequence[3][2=,3=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{\{ #1_{#2}\}}}{\ensuremath{\{ #1_{#2}, \eqsp #2 \in #3 \}}}}

\newcommandx{\sequencen}[2][2=n\in\N]{\ensuremath{\{ #1_n, \eqsp #2 \}}}

\newcommandx\dsequence[4][3=,4=]{\ensuremath{ ((#1_{#3}, #2_{#3}))_{#3 \in #4}}}


\newcommand{\wrt}{w.r.t.}
\newcommand{\Withoutlog}{w.l.o.g.}
\def\iid{\text{i.i.d.}}
\def\ifof{if and only if}
\def\eg{e.g.}

\def\Leb{\operatorname{Leb}}
\def\Id{\operatorname{I}}

\def\pdftarget{\target}

\def\Psemigroup{\mathbf{P}}
\def\barbdriftmalabeta{\bar{b}_{\bareta,\bgamma}^{(\beta)}}
\def\barbdriftmala{\bar{b}_{\bareta,\bgamma}^{\mathrm{M}}}
\def\varepsilonula{\varepsilon}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\def\tGamma{\tilde{\Gamma}}
\def\Phibf{\mbox{\protect\boldmath$\Phi$}}
\newcommand{\parenthese}[1]{\left(#1 \right)}
\def\tbdriftulatGamma{\tilde{b}_{\tGamma_{1/2}}^{\mathrm{U}}}


\def\target{\pi}
\def\normconst{\operatorname{Z}}
\def\pdfproposal{\proposal}
\def\proposal{\lambda}
\def\proposalbase{\varphi}
\def\pdfproposalbase{\varphi}
\def\ExKernel{\mathsf{Q}}
\def\eProposal{\bar{\proposal}_N}
\def\kernel{\mathsf{K}}
\def\kernelMTM{\mathsf{T}}
\def\fwdker{\mathsf{M}}
\def\fwddens{m}
\def\fwdkerwlat{\mathsf{N}}
\def\bckkerwlat{\breve{\mathsf{N}}}
\def\bckker{\mathsf{L}}
\def\bckdens{\mathsf{\ell}}
\def\Normal{\mathrm{N}}
\def\MALA{\operatorname{MALA}}
\def\bound{\mathrm{L}}
\def\epssmallisir{\epsilon_N}
\def\bisir{\mathrm{b}_N}
\def\driftconstisir{\kappa_N}
\def\rateisir{\tilde{\kappa}_N}


%
%=== MALA notations
%
\def\bfx{\mathbf{x}}
\def\bfy{\mathbf{y}}
\def\bfY{\mathbf{Y}}
\def\bfX{\mathbf{X}}
\def\bfB{\mathbf{B}}
\def\YrULA{Y}
\def\YrMALA{X}
\def\gaStep{\gamma}
\def\ZrGaussian{Z}
\def\bdriftula{b_{\bgamma}^{\mathrm{U}}}
\def\tbdriftula{\tilde{b}_{\bgamma}^{\mathrm{U}}}
\def\bdriftmala{b_{\bgamma}^{\mathrm{M}}}
\def\ray{K}
\def\rayula{\ray^{\mathrm{U}}}
\def\raymaladrift{\ray^{\mathrm{M}}}
\def\Veta{V}
\def\tCtt{\tilde{\mathtt{C}}}
\def\bGamma{\bar{\Gamma}}
\def\barA{\bar{A}}
\def\bareta{\bar{\eta}}



\def\constisir{c_N}
\def\disir{d_N}
\def\raten{\theta_N}
\def\MKP{{\rm P}}
\def\MKR{{\rm R}}
\def\MKQ{\mathsf{Q}}
\def\MKK{{\rm K}}
\def\dim{\mathsf{D}}



\newcommandx{\MKisir}[1][1=N]{\mathsf{P}_{#1}}
\def\Xset{\mathbbm{X}}
\def\Xsigma{\mathcal{X}}
\def\Eset{\mathbbm{E}}
\def\Esigma{\mathcal{E}}
\def\Zset{\mathbbm{Z}}
\def\Zsigma{\mathcal{Z}}
\def\Lset{\mathbbm{L}}
\def\Lsigma{\mathcal{L}}
\def\pdf{p.d.f.}

\newcommand{\chunk}[3]{#1_{#2:#3}}

\newcommand{\chunku}[3]{#1^{#2:#3}}
\newcommand{\chunkl}[3]{#1_{#2:#3}}
\newcommand{\chunkul}[5]{#1_{#2:#3}^{#4:#5}}
\newcommand{\chunkum}[4]{#1^{#2:#3 \setminus \{#4\}}}
\newcommand{\chunkulm}[6]{#1_{#2:#3}^{#4:#5 \setminus \{#4\}}}

\newcommand{\range}[1]{[#1]}
\def\biasconst{\upsilon}
\def\weightfunc{w}
\def\unormweight{\bar{\omega}}
\def\normweight{\omega}
\def\NormFactor{\Omega_N}
\def\rejukernel{\mathsf{R}}
\newcommandx{\XtryK}[1][1=N]{\mathsf{K}_{#1}}
\def\XtryKc{\mathsf{C}_N}
\def\dommeas{\mu}
\def\logit{\operatorname{logit}}
\newcommand{\jacop}[1]{\operatorname{J}_{#1}}

\def\isir{\ensuremath{\operatorname{i-SIR}}}
\def\XTryL{\texttt{X-Try Langevin}}
%\def\XTryM{\texttt{CiterSIR}}
\def\XTryM{\ensuremath{\operatorname{Ex^2MCMC}}}
\def\FlXTryM{\ensuremath{\operatorname{FlEx^2MCMC}}}

\def\gauss{\mathcal{N}}

\def\AXTryM{\texttt{CiterAIS}}
\def\PriorLatent{\Xi}
\newcommandx{\ePriorLatent}[1][1=N]{\bar{\Xi}_{#1}}
\def\PriorKernel{\mathsf{R}}
\def\PriorKerneldens{\mathsf{r}}
\def\SPriorLatent{\mathsf{S}}
\def\bPriorKernel{\breve{\mathsf{R}}}
\def\bPriorKerneldens{\breve{\mathsf{r}}}

%\newcommandx{\fwdtransf}[4][1=\gamma]{\mathsf{T}^{#1}_{#2,#3}(#4)}
%\newcommandx{\bcktransf}[4][1=\gamma]{\mathsf{G}^{#1}_{#2,#3}(#4)}
\newcommand{\fwdtransf}[3]{\mathsf{T}_{#1,#2}(#3)}
\newcommand{\bcktransf}[3]{\mathsf{G}_{#1,#2}(#3)}

\newcommand{\bcktransfwa}[2]{\mathsf{G}_{#1,#2}}
\newcommand{\AR}[3]{\alpha_{#1}(#2,#3)}
\newcommand{\bAR}[2]{\bar{\alpha}_{#1}(#2)}
\def\densgauss{\operatorname{g}}
\def\distrgauss{\mathcal{N}}
\def\eTarget{\bar{\target}_N}
\def\innov{w}
\def\accept{u}
\def\energy{\operatorname{U}}
\def\ESS{\operatorname{ESS}}
\def\Kprop{\operatorname{M}}

\def\unif{\operatorname{Unif}}
\def\True{\operatorname{True}}


\newcommand{\supnorm}[1]{| #1 |_{\infty}}

\newcommand{\KL}[2]{{\rm KL}(#1||#2)}
\newcommand{\KLhat}[2]{{\rm \widehat{KL}}(#1||#2)}


\def\partopopN{\boldsymbol{\Lambda}_N}
\def\eTarget{\boldsymbol{\varphi}_N}
\def\eTargetmarginx{\boldsymbol{\pi}_N}
\newcommandx{\targetkern}[1][1=N]{\Pi_{#1}}
\newcommandx{\utargetkern}[1][1=N]{\Gamma_{#1}}
\newcommandx{\MKisirjoint}[1][1=N]{\mathsf{\mathbf{P}}_{#1}}
\def\xijoint{{\boldsymbol{\xi}}}
\def\simiid{\overset{\text{i.i.d.}}{\sim}}


==> Local - (learned) Global Mixed Kernels/isir-proof.tex <==
\subsection{\isir\ and Multiple-try Metropolis (MTM) algorithm}
\label{subsec:isir-MTM}
In the MTM algorithm, $N$ \iid sample proposals $\{X^{i}_{k+1}\}_{i = 1}^N$ are drawn from a kernel $\kernelMTM(y, \cdot)$ in each iteration. In a second step, a sample $Y^*_{k+1}$ is selected with probability proportional to the weights (the exact expression of the weighting weights differs from ours, but this does not change the complexity of the algorithm). In a third step, $N-1$ \iid\ proposals are drawn from the kernel $\kernelMTM(Y^*_{k+1}, \cdot)$ and it is assumed that the move is $Y_{k+1}= Y^*_{k+1}$ with an \emph{generalised M-H} ratio, see~\citep[eq.~3]{liu2000multiple}. This step is bypassed in \isir, reducing the computational complexity by a factor of $2$.

\subsection{\isir\ as a systematic scan two-stage Gibbs sampler}
\label{subsec:two-stages-gibbs}
We analyze a slightly modified version of the {\isir} algorithm, with an extra randomization of the state position.
The $k$-th iteration is defined as follows. Given a state $Y_k \in \Xset$,
\begin{enumerate}[label=(\roman*),nosep,leftmargin=*]
\item draw $I_{k+1} \in \{1,\dots,N\}$ uniformly at random and set $X^{I_{k+1}}_{k+1}=Y_k$;
\item draw $\chunkum{X_{k+1}}{1}{N}{I_{k+1}}$ independently from the proposal distribution $\proposal$;
\item compute, for $i \in \{1, \dots, N\}$, the normalized importance weights
\[ \omega^i_{N,k+1} = \weightfunc(X^i_{k+1})/\sum_{\ell=1}^N \weightfunc(X^\ell_{k
+1});
\]
\item select $Y_{k+1}$ from the set $\chunku{X_{k+1}}{1}{N}$ by choosing $X_{k+1}^i$ with probability $\omega^i_{N,k+1}$.
\end{enumerate}
Thus, compared to the simplified \isir\ algorithm given in the introduction, the state is inserted uniformly at random into the list of candidates instead of being inserted at the first position. Of course, this change has no impact as long as we are interested in integrating functions that are permutation invariant with respect to candidates, which is the case throughout our work. Still, this randomization makes the analysis much more transparent.


In what follows, we show that {\isir} can be interpreted as a systematic-scan two-stage Gibbs sampler sampling, which alternately samples from the full conditionals of the extended target $\eTarget$, which is carefully defined below in terms of the state and candidate pool. Here we essentially follow the work of \cite{tjelmeland2004using,andrieu2010particle,andrieu2018uniform}. This is formalized by a dual representation of $\eTarget$, presented below in \Cref{thm:Gibbs:duality}, which provides the two complete conditionals in question.
We introduce the Markov kernel
\begin{equation}
\label{eq:definition-psiN}
\partopopN(y, \rmd \chunku{x}{1}{N}) = \frac{1}{N} \sum_{i=1}^N \delta_y(\rmd x^i) \prod_{j \ne i} \proposal(\rmd x^j)
\end{equation}
on $\Xset \times \Xsigma^{\varotimes N}$, which probabilistically describes the candidate selection operation in {\isir}.
Note that by construction, for each $y \in \Xset$, $\ell \in \{1, \dots, N\}$ and nonnegative measurable function $h: \Xset \to \rset^+$,
$$
\partopopN h(y) = \int \partopopN(y, \rmd \chunku{x}{1}{N}) h(x^\ell) = \left(1 - \frac{1}{N} \right) \proposal(h) + \frac{1}{N} h(y).
$$
Using the kernel $\partopopN$ we may now define properly the extended target $\eTarget$ as the probability law
\begin{equation}
\label{eq:extended-target}
\eTarget(\rmd (y, \chunku{x}{1}{N})) = \target(\rmd y) \partopopN(y, \rmd \chunku{x}{1}{N}) = \frac{1}{N} \sum_{i=1}^N \target(\rmd y)
\delta_y(\rmd x^i) \prod_{j \ne i} \proposal(\rmd x^j)
\end{equation}
on $(\Xset^{N + 1}, \Xsigma^{\varotimes (N + 1)})$. Note that since for every $A \in \Xsigma$, $\eTarget(\indi{A \times \Xset}) = \target(A)$, the target $\target$ coincides with the marginal of $\eTarget$ with respect to the state. Moreover, it is easily seen that $\partopopN$ provides the conditional distribution, under $\eTarget$, of the candidate pool given the state.
% Eric: this not well defined at this stage ! in the sense that, a.s., $\PP_{\sim \eTarget} (\chunku{X}{1}{N} \in \cdot \mid Y) = \partopopN(Y, \cdot )$.

On the other hand, using that $\target(\rmd y) \delta_y(\rmd x^i) = \weightfunc(x^i) \proposal(\rmd x^i) \delta_{x^i}(\rmd y) / \proposal(\weightfunc)$, the marginal distribution $\eTargetmarginx$ of $\eTarget$ with respect to $\chunku{x}{1}{N}$ is given by
\begin{equation} \label{eq:marginal-joint}
%\eTargetmarginx(\rmd \chunku{x}{1}{N}) = \frac{1}{N \proposal(\weightfunc)} \left( \sum_{i=1}^N \weightfunc(x^i) \right) \prod_{j=1}^N \proposal(\rmd x^j).
\eTargetmarginx(\rmd \chunku{x}{1}{N}) = \frac{1}{\proposal(\weightfunc)} \utargetkern \1_\Xset(\chunku{x}{1}{N}) \prod_{j=1}^N \proposal(\rmd x^j) \eqsp,
\end{equation}
where we have set
\begin{equation}
\label{eq:def-utargetkern}
\utargetkern (\chunku{x}{1}{N}, \rmd y) = \sum_{i=1}^N \weightfunc(x^i) \delta_{x^i}(\rmd y) / N, \quad 
\targetkern(\chunku{x}{1}{N}, \rmd y) = {\utargetkern(\chunku{x}{1}{N}, \rmd y)}/{\utargetkern \1_{\Xset} (\chunku{x}{1}{N})}
\end{equation}
It is interesting to note that the marginal $\eTargetmarginx$ has a probability density function, proportional to $\utargetkern \1_\Xset(\chunku{x}{1}{N}) = \sum_{i=1}^N \weightfunc(x^i) / N$, with respect to the product measure $\proposal^{\varotimes N}$. Using \eqref{eq:marginal-joint}, we immediately obtain the following result.

\begin{theorem}[duality of extended target] \label{thm:Gibbs:duality}
For every $N \in \nsets$,
\[
\eTarget(\rmd (y, \chunku{x}{1}{N})) = \target(\rmd y) \partopopN(y,\rmd \chunku{x}{1}{N}) = \eTargetmarginx(\rmd \chunku{x}{1}{N}) \targetkern(\chunku{x}{1}{N}, \rmd y).
\]
\end{theorem}
Using this dual representation of $\eTarget$, \isir\ can be interpreted as a two-stage Gibbs sampler. Given the state $Y_k$, $N$ candidates $\chunku{X_{k+1}}{1}{N}$ are sampled from $\partopopN(Y_k, \cdot)$. In a second step, the next state $Y_{k+1}$ is sampled given the current candidates from $\targetkern(\chunku{X_{k+1}}{1}{N}, \cdot)$. The two-stages Gibbs sampler generates a Markov chain $\dsequence{Y}{\chunku{X}{1}{N}}[k][\nset]$ with Markov kernel
\begin{equation}
\label{eq:joint-kernel}
\MKisirjoint((y, \chunku{x}{1}{N}), C) = \int \partopopN(y,\rmd \chunku{\tilde{x}}{1}{N}) \targetkern(\chunku{\tilde{x}}{1}{N},\rmd \tilde{y}) \indi{C}(\rmd (y,\chunku{\tilde{x}}{1}{N}))  \eqsp, \quad C \in \Xsigma^{\otimes (N+1)}\eqsp.
\end{equation}
Note that the Markov kernel $\MKisirjoint(y, \chunku{x}{1}{N}, \cdot)$ does not depend on $\chunku{x}{1}{N}$, which means that only the state $Y_k$ needs to be stored from one iteration to another. Given a distribution $\xijoint$ on $(\Xset^{n+1},\Xsigma^{\otimes (n+1)})$, we denote by $\PP _\xijoint$ the distribution of the canonical Markov chain $\dsequence{Y}{\chunku{X}{1}{N}}[k][\nset]$ with kernel $\MKisirjoint$. With these notations, for any nonnegative measurable function $f: \Xset^{n+1} \to \rset$, we get, for $k \in \nsets$,
\begin{align}
\label{eq:definition-Mkisir-joint}
\CPE[\xijoint]{f(Y_{k},\chunku{X_{k}}{1}{N})}{\mcf_{k-1}}=
\int \MKisirjoint((Y_{k-1}, \chunku{X_{k-1}}{1}{N}), \rmd (y,\chunku{x}{1}{N})) f(\chunku{x}{1}{N})= \MKisirjoint f(Y_{k-1}, \chunku{X_{k-1}}{1}{N}) \eqsp.
\end{align}
The systematic scan two-stages Gibbs sampler is one of the MCMC algorithm structures that has given rise to many works. We summarize in the theorem below the important properties of this sampler; see \cite{liu1994covariance}, \cite[Chapter~9]{robert:casella:2013},  \cite{andrieu2016random} and the references therein.
\begin{theorem}
\label{theo:main-properties-deterministic-scan}
Assume that for any $y \in \Xset$, $\weightfunc(y) >0$. Then,
\begin{itemize}[leftmargin=*,nosep]
\item The Markov kernel $\MKisirjoint$ is Harris recurrent and ergodic with unique invariant distribution $\eTarget$.
\item The Markov kernel $\MKisir$ is reversible \wrt\ $\target$, Harris recurrent and ergodic.
\end{itemize}
\end{theorem}
The proof follows from \cite[Theorem~9.6, Lemma~9.11]{robert:casella:2013}.
The following theorem establishes the unbiasedness of the estimator $\targetkern f(\chunku{X}{1}{N})$ under $\eTarget$.
\begin{theorem} \label{thm:unbiasedness}
For every $N \in \nsets$ and $\target$-integrable function $f$,
$$
\pi(f):= \int \targetkern f(\chunku{x}{1}{N}) \eTargetmarginx(\rmd \chunku{x}{1}{N}) = \int \targetkern f(\chunku{x}{1}{N}) \pi(\rmd x^1) \prod_{j=2}^N \proposal(\rmd x^j) 
\eqsp.
$$
\end{theorem}
\begin{proof}
Using \eqref{eq:marginal-joint} we get
\begin{align}
\int \eTargetmarginx(\rmd \chunku{x}{1}{N}) \targetkern f(\chunku{x}{1}{N})
&=  \int \frac{1}{N \proposal(\weightfunc)} \sum_{\ell=1}^N \weightfunc(x^\ell) \targetkern f(\chunku{x}{1}{N}) \prod_{j=1}^N \proposal(\rmd x^j) \\
&= \frac{1}{N \proposal(\weightfunc)} \int \sum_{i=1}^N \weightfunc(x^i) f(x^i) \prod_{j=1}^N \proposal(\rmd x^j)= \target(f),
\end{align}
and the first identity follows. The second identity stems from the fact that the function $\targetkern f(\chunku{x}{1}{N})$ is invariant under permutation.
\end{proof}

==> Local - (learned) Global Mixed Kernels/proof_adapt.tex <==
\def\Vset{\mathbb{U}}
\def\Vsigma{\mathcal{U}}
\def\Eset{\mathbb{E}}
\def\Esigma{\mathcal{E}}
\def\MCState{U}
\def\MCstate{u}
\def\MCNoise{E}
\def\MCnoise{e}
\def\borel{\mathcal{B}}
\def\Proj{\operatorname{Proj}}
\def\proj{{\operatorname{proj}}}
\def\targetadapt{\mu}
\def\driftfunc{V}
\def\propnoise{\rho}
The proof relies on results of stochastic approximation with Markovian dynamics; see  \cite{andrieu2005stability,andrieu2015stability}. For reader's convenience, before going into the details, we give an outline of the proof. The motivation of such algorithms is to find the roots of the function $h: \Theta \to \rset^q$, $\Theta \subset \rset^q$
\[
h(\theta) =  \int_{\Vset \times \Eset} H(\theta, \MCstate, \MCnoise) \targetadapt(\rmd \MCnoise) \propnoise_\theta( \rmd \MCnoise) \eqsp,
\]
for  families of functions $\{H(\theta, \MCstate, \MCnoise) : \Theta \times \Vset \times \Eset \rightarrow \Theta\}$, a family of probability distributions $\{\propnoise_\theta, \theta \in \Theta$ of $(\Eset,\Esigma)$ and a probability distribution $\targetadapt$ on a space $(\Vset,\Vsigma)$. These roots are not available analytically and a way of finding them numerically consists of considering the controlled Markov chain on $\left\{(\Theta \times \Vset)^{\nset},(\borel(\Theta) \otimes \Vsigma)^{\otimes \nset} \right\}$ initialized at some $(\theta_0,\MCState_0)= (\vartheta,\MCstate) \in \Theta \times \Vset$ and defined recursively for a sequence of stepsize $\sequence{\gamma}[i][\nset]$ by
\begin{equation}
\begin{split}
&\MCState_{i+1}  \sim P_{\theta_{i}}(\MCState_{i}, \cdot) \eqsp, \quad \MCNoise_{i+1} \sim \propnoise_{\theta_i} \\
&\theta_{i+1}=\theta_{i}+\gamma_{i+1} H(\theta_{i}, \MCState_{i+1},\MCNoise_{i+1}) \eqsp,
\end{split}
\end{equation}
where $\left\{P_{\theta}, \theta \in \Theta\right\}$ is a family of Markov kernels such that for each $\theta \in \Theta$, $\targetadapt P_\theta= \targetadapt$. The rationale for this recursion goes as follows. Let us first rewrite the Robbins-Monro recursion
\[
\theta_{i+1}= \theta_{i} + \gamma_{i+1} \{ h(\theta_{i}) + \xi_{i+1} \},
\]
where  $\xi_{i+1}= H(\theta_i,\MCState_{i+1},\MCNoise_{i+1})$  is referred to as the "noise". Therefore, $\{\theta_i\}$ is a noisy version of the sequence $\{\bar{\theta}_i\}$ defined as $\bar{\theta}_{i+1}= \bar{\theta}_i + \gamma_{i+1} h(\bar{\theta}_i)$. The convergence of such sequences has been studied by many authors, starting with \cite{metivier1987theoremes} under various conditions. A crucial step of such convergence analysis consists of assuming that the sequence $\{\theta_i\}$ remains bounded with probability 1 in a compact set of $\Theta$. This problem has traditionally can be circumvented by
means of modifications of the recursion. Indeed, one of the major difficulties
specific to the Markovian dynamic scenario is that $\{\theta_i\}$ governs the ergodicity of the controlled Markov chain $\{\MCState_i\}$  and that stability properties of $\{\theta_i\}$  require "good" ergodicity properties which might vanish whenever $\{\theta_i\}$ approaches $\partial \Theta$ often away from the roots of $h(\theta)$, resulting in instability. Most existing results rely on modifications of the updates designed to ensure a form of ergodicity
of $\{\xi_i\}$ which in turn ensures that $\{\theta_i\}$ inherits the stability properties of $\{\bar{\theta}_i\}$; see \eg\ \cite{andrieu2005stability,andrieu2014markovian} and the discussion in \cite[Section~3]{andrieu2015stability}. We follow here \cite{andrieu2014markovian}. Let $\{\mathcal{R}_i\}$ be a sequence of compact subsets of $\Theta$ and consider the recursion:
\begin{equation}
\begin{split}
&\MCState_{i+1} \sim P_{\theta_i}(\MCState_i,\cdot) \quad \MCNoise_{i+1} \sim \propnoise_{\theta_i} \\
&\theta_{i+1}^* = \theta_i + \gamma_{i+1} H(\theta_i,\MCState_{i+1},\MCNoise_{i+1})  \\
&\theta_{i+1}= \theta_{i+1}^* \indi{\mathcal{R}_{i+1}}(\theta^*_{i+1}) + \theta_{i+1}^{\operatorname{proj}} \indi{\mathcal{R}_{i+1}^c}(\theta_{i+1}^*)
\end{split}
\end{equation}
where, denoting $\mathcal{F}_i= \sigma( \MCState_0,\theta_j, j \leq i)$, $\theta_{i+1}^\proj$ is a random variable measurable w.r.t $\mathcal{F}_i \vee \sigma(\theta_{i+1}^*)$. Most common practical projection mechanisms include $\theta_{i+1}^{\operatorname{proj}}= \theta_i$, 'rejecting' an update outside the current feasible set, and $\theta_{i+1}^{\operatorname{proj}}= \Proj_{\mathcal{R}_{i+1}}(\theta^*_{i+1})$, where $\Proj$ is a measurable mapping $\Theta  \setminus \mathcal{R}_{i+1} \to \mathcal{R}_{i+1}$. In words, the expanding projections approach only ensures that $\theta_i$ is in a feasible set $\mathcal{R}_i$ but does not involve potentially harmful ‘restarts’ as is the case with the adaptive reprojection strategy of \cite{andrieu2005stability}.
We use the results in \cite{andrieu2014markovian} to show that the SA $\{\theta_i\}$ 'stays away' from $\partial \Theta$ with probability one for any initialization $(\theta_0,\MCstate) \in \mathcal{R}_0 \times \Vset$ under appropriate conditions on $\{H(\theta,\MCstate,\MCnoise), (\theta,\MCstate,\MCnoise) \in \Theta \times \Vset \times \Eset\}$, $\{ P_\theta, \theta \in \Theta\}$ and $\{\mathcal{R}_i\}$.
We denote throughout  the probability distribution associated to the process $\left(\theta_{i}, \MCState_{i}\right)_{i \geq 0}$ defined in Algorithm $1.1$ and starting at $\left(\theta_{0}, \MCState_{0}\right) \equiv(\theta, \MCstate) \in \Theta \times \Vset$ as $\PP_{\theta, \MCstate}(\cdot)$ and the associated expectation as $\PE_{\theta, \MCstate}[\cdot]$.
The approach developed in \cite{andrieu2014markovian} relies on the existence of a Lyapunov function $w: \Theta \rightarrow[0, \infty)$ for the recursion on $\theta$ and the subsequent proof that $\left\{w\left(\theta_{i}\right)\right\}$ is $\PP_{\theta, \MCstate}$-a.s. under some adequate level. For any $M>0$, we define the level sets $\mathcal{W}_{M}:=\{\theta \in \Theta: w(\theta) \leq M\}$.
Consider the following assumptions:
\begin{assumptionSA}
\label{assum:SA:stability-1}
There exists a continuously differentiable function $w: \Theta \rightarrow \coint{0, \infty}$ such that
\begin{enumerate}[label=(\roman*),leftmargin=*,nosep]
\item For all $\theta,\theta' \in \Theta$,
\[
\Vert \nabla w(\theta) - \nabla w(\theta') \Vert \leq C_{w} \Vert \theta - \theta' \Vert \eqsp.
\]
\item the projection sets are increasing subsets of $\Theta$, that is, $\mathcal{R}_{i} \subset \mathcal{R}_{i+1}$ for all $i \geq 0$, and
$$
\hat{\Theta}:=\bigcup_{i=0}^{\infty} \mathcal{R}_{i} \subset \Theta \eqsp,
$$
\item there exists a constant $M_{0}>0$ such that for any $\theta \in \mathcal{W}_{M_{0}}^{c} \cap \hat{\Theta}$
$$
\ps{\nabla w(\theta)}{h(\theta)} \leq 0
$$
\item the family of random variables $\left\{\theta_{i}^{\mathrm{proj}}\right\}_{i \geq 1}$ satisfies for all $i \geq 1$ whenever $\theta_{i}^{*} \notin \mathcal{R}_{i}$
$$
\theta_{i}^{\mathrm{proj}} \in \mathcal{R}_{i} \quad \text { and } \quad w\left(\theta_{i}^{\mathrm{proj}}\right) \leq w\left(\theta_{i}^{*}\right) \quad \PP_{\theta, \MCstate}-\as.
$$
\item there exists constants $ c \in \coint{0, \infty}$ and a non-decreasing sequence of constants $\zeta_{i} \in \coint{1, \infty}$ satisfying $\sup _{\theta \in \mathcal{R}_{i}}|\nabla w(\theta)| \leq c \zeta_{i}$ for all $i \geq 0$.
\end{enumerate}
\end{assumptionSA}
Hereafter, we denote the 'centred' version of  $\bar{H}(\theta,\MCstate,\MCnoise):=H(\theta, \MCstate,\MCnoise)-h(\theta)$. For the stability results, we shall introduce the following general condition on the noise sequence. In general terms, it is related to the rate at which $\left\{\theta_{i}\right\}$ may approach $\partial \hat{\Theta}$ in relation to the growth of $\Vert H(\theta, \MCstate, \MCnoise) \Vert$ and the loss of ergodicity of $P_{\theta}$.
\begin{assumptionSA}
\label{assum:SA:stability-2}
For any $(\theta, \MCstate) \in \mathcal{R}_{0} \times \Vset$ it holds that
\begin{enumerate}[label=(\roman*),leftmargin=*,nosep]
\item $\PP_{\theta, \MCstate}\left(\lim _{i \rightarrow \infty} \gamma_{i+1} \Vert\nabla w(\theta_{i})\Vert  \cdot \Vert H(\theta_{i}, \MCState_{i+1},\MCNoise_{i+1}) \Vert =0 \right)=1$,
\item $\PE_{\theta, \MCstate}\left[\sum_{i=0}^{\infty} \gamma_{i+1}^{2}\Vert H(\theta_{i}, \MCState_{i+1},\MCNoise_{i+1}) \Vert^2 \right]<\infty$,
\item $\PE_{\theta, \MCstate}\left[\sup _{k \geq 0}\left|\sum_{i=0}^{k} \gamma_{i+1}\ps{\nabla w(\theta_{i})}{ \bar{H}(\theta_{i}, \MCState_{i+1},\MCNoise_{i+1})} \right|\right]<\infty$.
\item $\lim _{\theta \rightarrow \partial \hat{\Theta}} w(\theta)=\infty$
\end{enumerate}
\end{assumptionSA}
\begin{theorem}
Assume \Cref{assum:SA:stability-1}-\Cref{assum:SA:stability-2}. Then, for any $(\theta, \MCstate) \in \mathcal{R}_{0} \times \mathrm{\MCState}$
$$
\PP_{\theta, \MCstate}\left(\limsup _{i \rightarrow \infty} w\left(\theta_{i}\right)<\infty\right)=1 .
$$
\end{theorem}
\begin{proof}
The proof is a simple adaptation of \cite[Theorem~2.5]{andrieu2014markovian}.
\end{proof}

The condition $\lim _{\theta \rightarrow \partial \hat{\Theta}} w(\theta)=\infty$ is weakened in \cite[Section~2.2]{andrieu2014markovian}. Verifiable conditions implying \Cref{assum:SA:stability-2} are given in
\cite[Section~3, Condition~3.1]{andrieu2014markovian}. They are summarized in the next assumption.
In the assumptions below, it is implicitly assumed that \Cref{assum:SA:stability-1} holds with constants $\left(\zeta_{i}\right)_{i \geq 0}$.

We denote $\tilde{H}(\theta,\MCstate)= \int \bar{H}(\theta,\MCstate,\MCnoise) \propnoise(\rmd \MCnoise)$ and we consider the following assumptions:
\begin{assumptionSA}
\label{assum:SA:stability-3}
 For all $\theta \in \hat{\Theta}$, the solution $g_{\theta}: \Vset \rightarrow \Theta$ to the Poisson equation $g_{\theta}(\MCstate)-P_{\theta} g_{\theta}(\MCstate) \equiv \tilde{H}(\theta, \MCstate)$ exists and for all $i \geq 0$ the step size $\Gamma_{i+1}$ is independent of $\mathcal{F}_{i}$ and $\MCState_{i+1}$. Moreover, there exist a measurable function $\driftfunc: \Vset \rightarrow[1, \infty)$ and constants $c<\infty, \beta_{H}, \beta_{g} \in[0,1 / 2]$ and $\alpha_{g}, \alpha_{H}, \alpha_{\driftfunc} \in[0, \infty)$ such that for all $(\theta, \MCstate) \in \mathcal{R}_{0} \times \Vset$
\begin{enumerate}[label=(\roman*),leftmargin=*,nosep]
\item $\sup _{\theta \in \mathcal{R}_{i}}|\tilde{H}(\theta, \MCstate)| \leq c \zeta_{i}^{\alpha_H} \driftfunc^{\beta_H}(\MCstate)$,
\item $\PE_{\theta, \MCstate}\left[\driftfunc\left(\MCState_{i}\right)\right] \leq c \zeta_{i}^{\alpha_\driftfunc} \driftfunc(\MCstate)$,
\item $\sup _{\theta \in \mathcal{R}_{i}}\left[\left|g_{\theta}(\MCstate)\right|+\left|P_{\theta} g_{\theta}(\MCstate)\right|\right] \leq c \zeta_{i}^{\alpha_{g}} \driftfunc^{\beta_{g}}(\MCstate)$,
\item $\sum_{i=1}^{\infty} \gamma_{i+1}\ \zeta_{i} \PE_{\theta, \MCstate}\left[\left|P_{\theta_{i}} g_{\theta_{i}}\left(\MCState_{i}\right)-P_{\theta_{i-1}} g_{\theta_{i-1}}\left(\MCState_{i}\right)\right|\right]<\infty$,
\item \label{item:stability-det-1} $\sum_{i=1}^{\infty} \gamma^2_{i} \zeta_{i}^{2 +2\left(\left(\alpha_{H}+\beta_{H} \alpha_{\driftfunc}\right) \vee\left(\alpha_{g}+\beta_{g} \alpha_{\driftfunc}\right)\right)}<\infty$,
\item \label{item:stability-det-2} $\sum_{i=1}^{\infty} \gamma_{i+1} \gamma_{i} \zeta_{i}^{\alpha_{H}+\alpha_{g}+\left(\beta_{H}+\beta_{g}\right) \alpha_\driftfunc}<\infty$,
\item \label{item:stability-det-3} $\sum^{\infty}\left|\gamma_{i+1}-\gamma_{i} \right| \zeta_{i}^{1+\alpha_{g}+\beta_{g} \alpha_{\driftfunc}}<\infty$.
\end{enumerate}
\end{assumptionSA}
For geometrically ergodic Markov chain, these conditions may be shown to boil down to "uniform-in-$\theta$" geometric ergodicity conditions and "smoothness" of the mapping $\theta \mapsto P_\theta$.
\begin{assumptionMC}
\label{assum:MC-1}
For any $r \in\ocint{0,1}$ and any $\theta \in \hat{\Theta}$, there exist constants $M_{\theta, r} \in \coint{0, \infty}$ and $\rho_{\theta, r} \in$ $(0,1)$, such that for any function $\|f\|_{\driftfunc^{r}}<\infty$
$$
\left|P_{\theta}^{k}f(\MCstate)-\targetadapt_\theta(f)\right| \leq \driftfunc^{r}(\MCstate)\|f\|_{\driftfunc^{r}} M_{\theta, r} \rho_{\theta, r}^{k}
$$
for all $k \geq 0$ and all $\MCstate \in \Vset$. Moreover, it holds that
$\sup _{\theta \in \mathcal{R}_{i}} M_{\theta, r} \leq c_{r} \zeta_{i}^{\alpha_{M}} \quad$ and $\quad \sup _{\theta \in \mathcal{R}_{i}}\left(1-\rho_{\theta, r}\right)^{-1} \leq c_{r} \zeta_{i}^{\alpha_{\rho}}$.
\end{assumptionMC}

\begin{assumptionMC}
\label{assum:MC-2}
For any $\theta, \theta^{\prime} \in \hat{\Theta}$, there exist a constant $D_{\theta, \theta^{\prime}, r} \in[0, \infty)$ and a constant $\beta_{D} \in(0, \infty)$ independent of $\theta, \theta^{\prime}$ and $r$ such that for any function $\|f\|_{\driftfunc^{r}}<\infty$
$$
\left\|P_{\theta} f-P_{\theta^{\prime}} f\right\|_{\driftfunc^{r}} \leq\|f\|_{\driftfunc^{r}} D_{\theta, \theta^{\prime}, r}\left|\theta-\theta^{\prime}\right|^{\beta_{D}} .
$$
Moreover, $\sup _{\left(\theta, \theta^{\prime}\right) \in \mathcal{R}_{i}^{2}} D_{\theta, \theta^{\prime}, r} \leq c_{r}^{D} \zeta_{i}^{\alpha_{D}}$ for some constant $c_{r}^{D} \in[0, \infty)$ depending only on $r \in(0,1]$
\end{assumptionMC}


\begin{assumptionMC}
\label{assum:MC-3}\Cref{assum:SA:stability-3}-(i) and (ii) hold with constants $\alpha_{H}, \beta_{H}$ and $\alpha_{\driftfunc}$, and there exist constants $c<\infty, \alpha_{\Delta} \in[0, \infty)$ and $\beta_{\Delta}>0$ such that
$$
\sup _{\left(\theta, \theta^{\prime}\right) \in \mathcal{R}_{i}^{2}}\left\|\tilde{H}(\theta, \cdot)-\tilde{H}\left(\theta^{\prime}, \cdot\right)\right\|_{\driftfunc^{\beta_{H}}} \leq c \zeta_{i}^{\alpha_{\Delta}}\left|\theta-\theta^{\prime}\right|^{\beta_{\Delta}} .
$$
\end{assumptionMC}
Up to this point, we have only considered the stability of the stochastic approximation process
with expanding projections. Indeed, after showing the stability we know that the projections can
occur only finitely often (almost surely), and the noise sequence can typically be controlled. Given this, the stochastic approximation literature provides several alternatives to show the convergence; see \cite{kushner2003stochastic,borkar2009stochastic}. We formulate below a convergence result following from \cite{andrieu2005stability}.
\begin{assumptionSA}
\label{assum:cvgce}
The set $\Theta \subset \mathbb{R}^{d}$ is open, the mean field $h: \Theta \rightarrow \mathbb{R}^{d}$ is continuous, and there exists a continuously differentiable function $\hat{w}: \Theta \rightarrow\coint{0, \infty}$ such that
\begin{enumerate}[label=(\roman*),leftmargin=*,nosep]
\item there exists a constant $M_{0}>0$ such that
$$
\mathcal{L}:=\{\theta \in \Theta:\ps{\nabla \hat{w}(\theta)}{h(\theta)}=0\} \subset\left\{\theta \in \Theta: \hat{w}(\theta)<M_{0}\right\}
$$
\item there exists $M_{1} \in\left(M_{0}, \infty\right]$  such that $\left\{\theta \in \Theta: \hat{w}(\theta) \leq M_{1}\right\}$  is compact.
\item for all $\theta \in \Theta \setminus \mathcal{L}$, the inner product $\ps{\nabla \hat{w}(\theta)}{ h(\theta)}<0$ and the closure of $\hat{w}(\mathcal{L})$ has an empty interior.
\end{enumerate}
\end{assumptionSA}



\begin{theorem}
Assume \Cref{assum:cvgce} holds, and let $\mathcal{K} \subset \Theta$ be a compact set intersecting $\mathcal{L}$,
that is, $\mathcal{K} \cap \mathcal{L} \neq \varnothing$. Suppose that $\left(\gamma_{i}\right)_{i \geq 1}$ is a sequence of non-negative real numbers satisfying $\lim _{i \rightarrow \infty} \gamma_{i}=0$ and $\sum_{i=1}^{\infty} \gamma_{i}=\infty$. Consider the sequence $\left(\theta_{i}\right)_{i \geq 0}$ taking values in $\Theta$ and defined through the recursion $\theta_{i}=\theta_{i}-1+\gamma_{i} h\left(\theta_{i-1}\right)+\gamma_{i} \varepsilon_{i}$ for all $i \geq 1$, where $\left(\varepsilon_{i}\right)_{i \geq 1}$ take values in $\mathbb{R}^{d}$.
If there exists an integer $i_{0}$ such that $\left\{\theta_{i}\right\}_{i \geq i_{0}} \subset \mathcal{K}$ and $\lim _{m \rightarrow \infty} \sup _{n \geq m}\left|\sum_{i=m}^{n} \gamma_{i} \varepsilon_{i}\right|=0$, then $\lim _{n \rightarrow \infty} \inf _{x \in \mathcal{L} \cap \mathcal{K}}\Vert\theta_{n}-x\Vert=0 .$
\end{theorem}
We have now all the necessary elements to prove \Cref{thm:KL-simplified}. For simplicity, we set
$\alpha_k = \alpha_\infty$ for any $k \in \nset$ and $\gamma_k= 1 / (1 + k)^{\iota}$ where $\iota \in \ocint{1/2,1}$.
In this case, the state space is $\Vset= \Xset^M$ and $\Eset= \Zset^{(N-1) \cdot M}$, $\MCState_k= (Y_k[j])_{j=1}^M$, $\MCNoise_k= (\chunku{Z_k}{2}{N}[j])_{j=2}^N$. 
With $\MCstate= (y[j])_{j=1}^M$  and $\MCnoise= (\chunku{z}{2}{N}[j])_{j=1}^M$, 
$H(\theta,\MCstate,\MCnoise)$ is given by
\[
H(\theta,\MCstate)= M^{-1} \sum_{mj=1}^N \{\alpha_\infty H^f(\theta,y[j],\chunku{z}{2}{N}[j]) + (1-\alpha_\infty) H^b(\theta,\chunku{z}{2}{N}[j]) \} \eqsp.
\]
where $H^f$ and $H^b$ are defined respectively in \eqref{eq:fwdKL} and \eqref{eq:bwdKL}.
In this case, the Markov kernel $P_\theta$ is given for any nonnegative function $f$,
\[
P_{\theta,N} f(y[1],\dots,y[M])=  \int \prod_{j=1}^N \XtryK[\theta,N](y[j],\rmd \tilde{y}[j])  f(\tilde{y}[1],\dots,\tilde{y}[M]) \eqsp,
\]
and $\XtryK[\theta,N]$ is defined in \eqref{sec:coupling-with-local} with $\proposal \leftarrow \proposal_\theta$ and $\weightfunc \leftarrow \weightfunc_\theta$. 
By construction, for any $\theta \in \Theta$, $P_\theta$ has a unique stationary distribution which is given by
$\targetadapt = \target^{\otimes M}$.
Using \Cref{thm:unbiasedness}, and, for all $\theta \in \Theta$,
\[
H^f(\theta,\chunku{x}{1}{N})= \targetkern[\theta,N] [\nabla_\theta \log \proposal_\theta](\chunku{x}{1}{N})
\]
we get that
\[
h(\theta)= - \alpha_\infty \nabla_\theta \KL{\target}{\proposal_\theta} - (1-\alpha_{\infty}) \nabla_\theta \KL{\proposal_\theta}{\target} \eqsp.
\]
Recall that $\Theta= \rset^q$.  To check \Cref{assum:SA:stability-1}, we set
\begin{equation}
w(\theta)= \alpha_\infty  \KL{\target}{\proposal_\theta} - (1-\alpha_{\infty})  \KL{\proposal_\theta}{\target} \eqsp,  \text{for $\theta \in \Theta$}.
\end{equation}
and for $i \in \nset$, $\zeta_i= \log(i+1)$. The subset $\mathcal{R}_i$ is a ball centered at $0$ and of radius $r_i$ where $r_i$ is chosen so that $\sup_{\| \theta \|\leq r_i} \nabla w(\theta) \| \leq c \zeta_i$ (such $r_i$ exists using \Cref{assum:condition-gradient}).  
It is easily checked that  \Cref{assum:SA:stability-1} is satisfied thanks to \Cref{assum:condition-gradient} (note in particular that $\nabla w$ is globally Lipshitz under the stated conditions). Conditions \Cref{assum:SA:stability-3}-\ref{item:stability-det-1}-\ref{item:stability-det-2}-\ref{item:stability-det-3} are automatically satisfied.

We consider the drift function for the Markov kernel $P_{\theta,N}$
\begin{equation}
\label{eq:drift-function}
\driftfunc(y[1],\dots,y[M])= \sum_{i=1}^M V(y[i]) 
\end{equation}
where $V$ is the drift function in \Cref{assum:rejuvenation-kernel}. \Cref{assum:MC-1} follows from \Cref{theo:main-geometric-ergodicity}  under \Cref{assum:independent-proposal-strengthen}. It is important to note that it is essential to have explicit controls on the drift and reduction conditions here. Conditions \Cref{assum:MC-2} and \Cref{assum:MC-2} follow from \Cref{assum:condition-gradient}. The precise tuning of constants is done along the same lines as \cite[Section~5.3]{andrieu2014markovian}. 

==> Local - (learned) Global Mixed Kernels/sec_adaptive.tex <==
%% Outline
% Performance of IS based sampling controlled by \weightfunc = ...
% Natural to try to improve the proposal to match the target, tradition of adaptive MCMC.
% Describe the concept
% Even more so with deep generative models, flexibility could make us hope to closely match target, in particular normalizing flows.
%
\vspace{-2mm}
The performance of proposal-based samplers depends on the distribution of importance weights which is related to the similarity of the proposal and target distributions\footnote{more specifically, it depends on the the quantities appearing in \Cref{assum:independent-proposal}, namely, the maximum of the importance weight on a level set of the drift function for the local kernel $\rejukernel$ and the variance of the importance weights under the proposal}.
Therefore, yet another strategy to improve sampling performance is to select the proposal distribution $\proposal$ from a family of parameterized distributions $\left\{\proposal_{\theta}\right\}$ and fit the parameter $\theta \in \Theta = \rset^q$ to the target $\target$, for example, by minimizing a Kullback-Leibler divergence (KL) \cite{Parno2018, albergo:2019, Naesseth2020} or matching moments \cite{Pompe2020}. In \emph{adaptive MCMCs}, parameter adaptation is performed along the MCMC run  \cite{andrieu2006ergodicity,andrieu2008tutorial,roberts2009examples}. In this section we propose an adaptive version of \XTryM, which we call \FlXTryM.


\textbf{Normalizing flow proposal.}
A flexible way to parameterize proposal distributions is to combine a tractable distribution $\proposalbase$ with an invertible parameterized transformation. Let $T: \Xset \mapsto \Xset$ be a $\rmc^1$ diffeomorphism. We denote by $\pushforward[T][\proposalbase]$ the push-forward of $\proposalbase$ under $T$, that is, the distribution of $X=T(Z)$ with $Z\sim\proposalbase$. Assuming that $\proposalbase$ has a p.d.f. (also denoted $\pdfproposalbase$), the corresponding push-forward density (w.r.t. the Lebesgue measure) is given by $\pdfproposal_T(y) = \pdfproposalbase\bigl(T^{-1}(y)\bigr) \jacop{T^{-1}}(y)$, where $\jacop{T}$ denotes the Jacobian determinant of $T$. The parameterized family of diffeomorphisms $\{T_\theta\}_{\theta \in \Theta}$ defines a family of distributions $\{\pdfproposal_{T_\theta}\}_{\theta \in \Theta}$, denoted for simplicity as $\{\pdfproposal_\theta\}_{\theta \in \Theta}$.
This construction is called a \emph{normalizing flow} (NF) and a great deal of work has been devoted to ways of parameterizing invertible flows $T_{\theta}$ with neural networks; see~\citep{kobyzev2020normalizing,papamakarios2019normalizing} for reviews.

\textbf{Simultaneous learning and sampling.} {As with adaptive MCMC methods, the parameters of a NF proposal are learned for the global proposal during sampling, see also \cite{Gabrie2021}.} We work with $M$ copies of the Markov chains $\{(Y_k[j], \chunku{X_k}{1}{N}[j])\}_{k \in \nsets}$ indexed by $j \in \{1,\dots, M \}$. At each step $k \in \nsets$, each copy is sampled as in \XTryM~using the NF proposal, independently from the other copies, but conditionally to the the current value of the parameters $\theta_{k-1}$.
% , \ie\
% \begin{equation}
%     X_k^1[j]= Y_{k-1}[j] \, \text{ and } \, X_k^{\ell}[j] = T_{\theta_{k-1}}(Z_k^{\ell}[j]), \ell \in \{2,\dots,N\} \, \text{ where } \, \{ \chunku{Z}^{2:N}_k[j] \} \simiid \proposalbase.
% \end{equation}
We then adapt the parameters by taking steps of gradient descent on a convex combination of the \emph{forward} KL, $\KL{\pdftarget}{\pdfproposal_\theta} = \int_{} \pdftarget(x) \log(\pdftarget(x)/\pdfproposal_\theta(x)) \rmd x$ and the backward KL  $  \KL{\pdfproposal_\theta}{\pdftarget} = \int \pdfproposal_\theta(x) \log (\pdftarget(x)/\pdfproposal_\theta(x)) \rmd x = \int \pdfproposalbase(z) \log \weightfunc_\theta \circ T_\theta(z)  \rmd z$.
Let $\sequence{\gamma}[k][\nset]$ be a sequence of nonnegative stepsizes and $\sequence{\alpha}[k][\nset]$ be a nondecreasing sequence in $\ccint{0,1}$ with $\alpha_{\infty}= \lim_{k \to \infty} \alpha_k$.
The update rule is $\theta_k= \theta_{k-1} + \gamma_k M^{-1} \sum_{j=1}^M  H(\theta_{k-1},\chunku{X_k}{1}{N}[j],\chunku{Z_k}{2}{N}[j])$ where  $H(\theta,\chunku{x}{1}{N},\chunku{z}{2}{N})= \alpha_k H^{f}(\theta,\chunku{x}{1}{N})+
(1-\alpha_k) H^b(\theta,\chunku{z}{2}{N})$ with
\begin{align}
\label{eq:fwdKL}
H^{f}(\theta,\chunku{x}{1}{N}) &=  \sum\nolimits_{\ell=1}^N \frac{\weightfunc_{\theta}(x^{\ell})}{\sum\nolimits_{i=1}^N \weightfunc_{\theta}(x^i)} \nabla_{\theta} \log \pdfproposal_{\theta}(x^{\ell})  \eqsp, \quad \weightfunc_\theta(x)= \pdftarget(x)/ \pdfproposal_\theta(x)\eqsp, \\
\label{eq:bwdKL}
H^b(\theta,\chunku{z}{2}{N})&= 
 - \frac{1}{N-1} \sum\nolimits_{\ell=2}^N \{ \nabla_\theta \log \pdftarget \circ T_\theta(z^\ell) + \nabla_\theta \log \jacop{T_\theta} (z^{\ell}) \}\eqsp.
\end{align}
Note that we use a Rao-Blackwellized estimator of the gradient of the forward KL \eqref{eq:fwdKL} where we fully recycle all the $N$ candidates sampled at each iteration of \isir. The quality of this estimator is expected to improve along the iterations $k$ of the algorithm as the variance of importance weights decreases as the proposal improves. Note also that using only gradients from the backward KL \eqref{eq:bwdKL} is prone to mode-collapse \cite{Parno2018,Noe2019,Naesseth2020,Gabrie2021}, hence the need for also using gradients from the forward KL $H^{f}(\theta,\chunku{x}{1}{N})$, which requires the simultaneous sampling from $\target$. {See also \Cref{app:subsec:mixture-highd} for further discussions.}
{The \FlXTryM\ algorithm is summarized in \Cref{alg:NF-X-Try-MCMC}.} 

Since the parameters of the Markov kernel $\theta_{k}$ are updated using samples $\chunku{X_k}{1}{N}$ from the chain, $\dsequence{Y}{\chunku{X}{1}{N}}[k][\nset]$ is no longer Markovian. This type of problems has been considered in \cite{metivier1987theoremes,benveniste1990adaptive,gu1998stochastic,andrieu2005stability} and to prove convergence of the strategy we need to strengthen assumptions compared to the previous section.
\begin{assumption}
\label{assum:condition-gradient}
There exists a function $W: \Xset \to \rset_+$ such that $\proposalbase(W^2)= \int W^2(z) \proposalbase(\rmd z) < \infty$, and a constant $L < \infty$ such that, for all $\theta, \theta' \in \Theta$ and $z \in \Xset$, $\Vert \nabla_\theta \log \target \circ T_\theta(z) - \nabla_\theta \log \target \circ T_{\theta'}(z)\Vert \leq L \| \theta - \theta' \| W(z)$ and $ \Vert \nabla_\theta \log \jacop{T_\theta} (z) - \nabla_\theta \log \jacop{T_{\theta'}} (z) \Vert \leq L \norm{\theta - \theta'} W(z)$.
\end{assumption}
\begin{assumption}
\label{assum:independent-proposal-strengthen}
(i) For all $d \geq d_{\rejukernel}$, $\weightfunc_{\infty, d}= \sup_{\theta \in \Theta} \sup_{x\in\msv_d} \weightfunc_\theta(x) / \proposal_\theta(\weightfunc_\theta) < \infty$ and (ii) $\sup_{\theta \in \Theta} \PVar_{\proposalbase}(\weightfunc_\theta \circ T_\theta)/ \{ \proposal_\theta(\weightfunc_\theta) \}^2 < \infty$.
\end{assumption}
\Cref{assum:condition-gradient} is a continuity condition on the NF push-forward density \wrt~its parameters $\theta$. \Cref{assum:independent-proposal-strengthen} implies that the Markov kernel $\XtryK[N,\theta] = \MKisir[N,\theta] \rejukernel$ satisfies a drift and minorization condition uniform in $\theta$.
\begin{theorem}[simplified]
\label{thm:KL-simplified}
Assume \Cref{assum:rejuvenation-kernel}-\Cref{assum:condition-gradient}-\Cref{assum:independent-proposal-strengthen} and that $\sum_{k=0}^\infty \gamma_k = \infty$, $\sum_{k=0}^{\infty} \gamma_k^2 < \infty$ and $\lim_{k \to \infty} \alpha_k= \alpha_\infty$. Then, w.p. 1, the sequence $\sequence{\theta}[k][\nset]$ converges to the set
$\{\theta \in \Theta,  0 = \alpha_\infty \nabla \KL{\target}{\proposal_\theta} + (1-\alpha_\infty) \nabla \KL{\proposal_\theta}{\target} \}$.
\end{theorem}
\Cref{thm:KL-simplified} proves the convergence of the learning of parameters $\theta$ to a stationary point of the loss. The proof is postponed to \Cref{sec:thm:KL-simplified}.
Note that once the proposal learning has converged, $\FlXTryM$ boils back to $\XTryM$ with a fixed learned proposal. 
Our experiments show that
adaptivity can significantly speed up mixing for \isir, especially for distributions with complex geometries and that the addition of a rejuvenation kernel
further improves samples quality.

{
\input{algo_flex}
}

==> Local - (learned) Global Mixed Kernels/sec_intro.tex <==

% In this paper,
We consider the setting where a target distribution $\target$ on a measurable space $(\Xset,\Xsigma)$ is known up to a normalizing constant and one tries to estimate the expectations of some function $f : \Xset \to \rset$ with respect to $\target$. Examples include the extraction of Bayesian statistics from posterior distributions derived from observations as well as the computation of observables of a physical system $x \in \Xset$ under the Boltzmann distribution with non-normalized density $\pdftarget(x)= \rme^{- \beta U(x)}$ for the energy function $U$ at the inverse temperature $\beta$.


A common strategy to tackle this estimation is to resort to Markov chain Monte Carlo algorithms (MCMCs). The MCMC approach aims to simulate a realization of a time-homogeneous Markov chain $\sequence{Y}[n][\nset]$, such that the distribution of the $n$-th iterate $Y_n$ with $n \to \infty$ is arbitrarily close to $\target$, regardless of the initial distribution of $Y_0$. In particular, the Metropolis-Hastings kernel (MH) is the cornerstone of MCMC simulations, with a number of successful variants following the process of a \emph{proposal} step followed by an \emph{accept/reject} step (see e.g. \cite{robert:2015:mh}). In large dimensions, proposal distributions are typically chosen to generate local moves that depend on the last state of the chain in order to guarantee an admissible acceptance rate. However, local samplers suffer from long mixing times as
% , especially in large dimension. 
exploration is inherently slow, and mode switching, when there is more than one, can be extremely infrequent.

On the other hand, independent proposals are able to generate more global updates, but they are difficult to design. Developments in deep generative modelling, in particular versatile autoregressive and normalising flows \cite{kingma:2016:aif,huang:2018:neural_aif,dinh:2016,papamakarios2019normalizing}, spurred efforts to use learned probabilistic models to improve the exploration ability of MCMC kernels. Among a rapidly growing body of work, references include \cite{Hoffman2019, albergo:2019, Nicoli2020, Gabrie2021, Hackett2021}. While these works show that global moves in a number of practical problems can be successfully informed by machine learning models, it remains the case that the acceptance rate of independent proposals decreases dramatically with dimensions -- except in the unrealistic case that they perfectly reproduce the target. This is a well-known problem in the MCMC literature \cite{Bengtsson:2008:Curse,Bickel:2008:obstacle,agapiou2017importance}, and it was recently noted that deep learning-based suggestions are no exception in works focusing on physical systems \cite{DelDebbio2021,Mahmoud2022}.

In this paper we focus on the benefits of combining local and global samplers. Intuitively, local steps interleaved between global updates from an independent proposal (learned or not) increase accuracy by allowing accurate sampling in tails that are not usually well handled by the independent proposal. Also, mixing time is usually improved by the local-global combination, which prevents long chains of consecutive rejections. Here we focus on a global kernel of type iterative-sampling importance resampling (\isir) \citep{tjelmeland2004using,andrieu2010particle,andrieu2018uniform}. This kernel uses multiple proposals in each iteration to take full advantage of modern parallel computing architectures. For local samplers, we consider common techniques such as Metropolis Adjusted Langevin (MALA) and Hamiltonian Monte Carlo (HMC). We call this combination strategy Explore-Exploit MCMC (\XTryM) in the following.

\vspace{-2mm}
\paragraph{Contributions} The main contributions of the paper are as follows:
\begin{itemize}[leftmargin=*,noitemsep]
\vspace{-2mm}
\item We provide theoretical bounds on the accuracy and convergence speed of \XTryM\ strategies. In particular, we prove $V$-uniform geometric convergence of \XTryM\ under assumptions much milder than those required to prove uniform geometric ergodicity of the global sampler \isir~alone. %We also evaluate the relative improvement of the mixing time when local and global moves are used synergetically.
\item We {provide convergence guarantees for} an adaptive version of the strategy, called \FlXTryM, which involves learning an efficient proposal while  sampling, as in adaptive MCMC.
\item We perform a numerical evaluation of \XTryM\ and \FlXTryM\ for various sampling problems, including sampling GANs as energy-based models. The results clearly show the advantages of the {combined} approaches compared to purely local or purely global MCMC methods.
\end{itemize}
\vspace{-3mm}
\paragraph{Notations} Denote $\nsets = \nset \setminus \{0\}$. For a measurable function $f: \Xset \mapsto \rset$, we define $\supnorm{f} = \sup_{x \in \Xset}|f(x)|$ and $\target(f) := \int_{\Xset} f(x) \target(\rmd x)$. For a function $V: \Xset \mapsto [1, \infty)$ we introduce the $V$-\emph{norm} of two probability measures $\xi$ and $\xi'$ on $(\Xset,\Xsigma)$, $\Vnorm{\xi - \xi'} \eqdef \sup_{|f(x)| \leq V(x)} |\xi(f) - \xi'(f)|$. If $V\equiv 1$, $\Vnorm [1]{\cdot}$ is equal to the total variation distance (denoted $\tvnorm{\cdot}$).




==> Local - (learned) Global Mixed Kernels/sec_numerics.tex <==
\vspace{-3mm}
\subsection{Synthetic examples}
\label{subsec:toy_examples}
\vspace{-3mm}
\paragraph{Multimodal distributions.}
Let us start with a toy example highlighting differences between purely global \isir, purely local MALA and \XTryM\ combining both. We consider sampling from a mixture of $3$ equally weighted Gaussians in dimension $d = 2$. In \Cref{fig:gaus_example_2d}, we compare single chains produced by each algorithms. The global proposal is a wide Gaussian, with pools of $N=3$ candidate. The MALA stepsize is chosen to reach a target acceptance rate of $\sim 0.67$. This simple experiment illustrates the drawbacks of both approaches: \isir\ samples reach all the modes of the target, but the chains often get stuck for several steps hindering variability. MALA allows for better local exploration of each particular mode, yet it fails to cover all the target support. Meanwhile, \XTryM\ retains the benefits of both methods, combining the \isir-based global exploration with MALA-based local exploration.
% \begin{figure}%[h]
% \centering
% \begin{subfigure}{0.8\textwidth}
% \centering
% % \captionsetup{justification=centering}
% \includegraphics[width=1.0\textwidth]{NeurIPS/figures/toy_samples_2d_gaus_tight.pdf}
% \end{subfigure}
% \caption{Single chain mixing visualization. -- Blue color levels represent the target 2d density. Random chain initialization is noted in black, $100$ steps are plotted per sampler: the size of each red dot corresponds to the number of consecutive steps the walkers remains at a given location. For MALA, we generate $300$ samples and choose each $3$-rd one for comparability. Note that the variance of the global proposal (dotted countour lines) should be relatively large to cover well all the modes. The step size of MALA also can not be increased much to keep reasonable acceptance ratio.}
% \label{fig:gaus_example_2d}
% \vspace{-3mm}
% \end{figure}

\vspace{-1mm}
{In larger dimensions, an adaptive proposal is necessary. In \Cref{app:subsec:mixture-highd} we show that \FlXTryM~can mix between modes of a $50d$ Gaussian mixture, provided that the rough location of all the modes is known and used to initialize walkers. We also stress the robustness of the on-the-fly training exploiting running MCMC chains to evaluate the forward KL term of the loss.}

To illustrate further the performance of the {combined kernel}, we keep the $2d$ target mixture model yet assigning the uneven weights $(2/3, 1/6, 1/6)$ to the $3$ modes. We start $M$ chains drawing from the initial distribution $\xi \sim \mathcal{N}(0,4\Id_d)$ and use the same hyper-parameters as above. In \Cref{fig:mog_burnin} we provide a simple illustration to the statement \eqref{eq:tv_dist_isir} and \Cref{theo:main-geometric-ergodicity}, namely we compare  the target density to the instantaneous distributions for each sampler propagating $\xi$ during burn-in steps. As MALA does not mix easily between modes, the different statistical weights of the different modes can hardly be rendered in few iterations and KL and TV distances stalls after a few iterations. \isir\ can visit the different modes, yet it does not necessarily move at each step which slows down its covering of the modes full support, which again shows in the speed of decrease of the TV and KL. Overcoming both of these shortcomings, \XTryM\ instantaneous density comes much closer to the target. Finally, \Cref{fig:mog_single_chain} evaluates the same metrics yet for the density estimate obtained with single chain samples after burn-in. Results demonstrate once again the superiority of \XTryM.
Further details on these experiments can be found in \Cref{supp:subsec:mixtures}.


% To compare the quality of the methods, we perform the following procedure
% \begin{itemize}[leftmargin=*,nosep]
%     \item starting with the initial distribution $\mathcal{N}(0,4\Id)$, we generate the trajectory $(X_1,\ldots,X_n)$ for different values of $n \in [25,800]$ for each of the compared methods (\isir\, MALA, \XTryM\ ). Sampler hyperparameters are the same as above, and the burn-in period equals $50$;
%     \item We perform the kernel density estimate (KDE) $\widehat{p}_{n}$ based on the observations $(X_1,\ldots,X_n)$, and compute the total variation distance between $\widehat{p}_{n}$ and the target density $p_{\beta}$, and the forward $\KL{\widehat{p}_{n}}{p_{\beta}}$. Then we average the results over $100$ independent runs of each sampler.
% \end{itemize}
% The results for each sampler are reported in \Cref{fig:kl_loss} and \Cref{fig:tv_loss}. We also provide a simple illustration to the statements of \eqref{eq:tv_dist_isir} and \Cref{theo:main-geometric-ergodicity}. Starting with the initial distribution $\xi \sim \mathcal{N}(0,4\Id)$, we sample $500$ independent chains of length $50$ for each of the compared methods. Upon these $500$ observations we build a KDE $\widehat{p}_{n}$ for the density corresponding to the distribution of $\xi \MKQ^{n}$ for different $n \in \{5,\ldots,50\}$ and $\MKQ$ corresponding to \isir\, MALA, or \XTryM\ . Then we compute the total variation distance between $\widehat{p}_{n}$ and the target density $p_{\beta}$. Corresponding plots are shown in \Cref{fig:tv_loss_parallel} and \Cref{fig:gaus_2d_loss_plots}. Note that \XTryM\ significantly outperforms the results of both MALA and \isir\ . Indeed, the inhomogeneous mixture model is complicated target for the Langevin-based methods. The MALA -generated trajectories tend to stay in one mode of the mixture \eqref{eq:gaus_mixture}, which decreases the reliability of the estimates, and requires to generate long trajectories even in case $d = 2$. At the same time, for \isir\ -type methods without local exploration moves it is hard to balance the time spent in one of the distribution modes.
% \vspace{-3mm}

\begin{figure}%[h]
\begin{minipage}{0.69\textwidth}
\centering
{\includegraphics[width=1.0\textwidth]{figures/toy_samples_2d_gaus_new.png}\label{fig:gaus_example_2d}}
\end{minipage}
\begin{minipage}{0.3\textwidth}
\centering
\begin{subfigure}{1.0\textwidth}
    \centering
    \captionsetup{justification=centering}
    \includegraphics[width=0.6\textwidth]{figures/3_gaussians/3_gauss_forward_KL_parallel.png}
    \vspace{-3mm}
    \caption{}
%     \caption{Forward KL between the parallel iterates}
%     \label{fig:tv_loss_parallel}
% \end{subfigure}
% \begin{subfigure}{0.24\textwidth}
    % \includegraphics[width=0.49\textwidth]{figures/3_gaussians/3_gauss_TV_parallel.png}
    % \caption{Parallel iterates burn-in ($M=500$ chains KDE)}
    \label{fig:mog_burnin}
\end{subfigure}
\\
\vspace{-1mm}
\begin{subfigure}{1.0\textwidth}
    \centering
    \captionsetup{justification=centering}
    \includegraphics[width=0.6\textwidth]{figures/3_gaussians/3_gauss_forward_KL.png}
    \vspace{-3mm}
    \caption{}
%       \caption{Forward KL}
%     \label{fig:kl_loss}
% \end{subfigure}
% \begin{subfigure}{0.24\textwidth}
    %   \includegraphics[width=0.49\textwidth]{figures/3_gaussians/3_gauss_TV.png}
    %   \caption{Single chain efficiency ($M=100$ average)}
    \label{fig:mog_single_chain}
\end{subfigure}
\label{fig:gaus_2d_loss_plots}
\end{minipage}
\vspace{-1mm}
\caption{(a) -- Single chain mixing visualization. -- Blue color levels represent the target 2d density. Random chain initialization is noted in black, $100$ steps are plotted per sampler: the size of each red dot corresponds to the number of consecutive steps the walkers remains at a given location. %For MALA, we generate $300$ samples and choose each $3$-rd one for comparability. 
Note that the variance of the global proposal (dotted countour lines) should be relatively large to cover well all the modes. %The step size of MALA also can not be increased much to keep reasonable acceptance ratio.\\
(b - c) -- Inhomogeneous 2d Gaussian mixture. -- Quantitative analysis during burn-in of parallel chains (b, $M=500$ chains KDE) and for after burn-in for single chains statistics (c, $M=100$ average).}
\vspace{-5mm}
\end{figure}
\vspace{-4mm}
\paragraph{Distributions with complex geometry.}
Next, we turn to highly anisotropic distributions in high dimensions. Following \cite{neal:slice:2003} and \cite{haario1999banana}, we consider the \emph{funnel} and the \emph{banana-shape} distributions. We remind densities in \Cref{supp:subsec:complex-geometry} along with providing experiments details. For $d \in [10; 200]$, we run \isir, MALA, \XTryM, \FlXTryM, adaptive \isir~ (using the same proposal as \FlXTryM, but without interleaved local steps) and the versatile sampler NUTS~\cite{hoffman2014no} as a baseline. Here the parameter adaptation for $\FlXTryM$ is performed in a pre-run and parameters are frozen before sampling.
% to sample $1000$ points.
For the adaptive samplers, a simple RealNVP-based normalizing flow \cite{dinh:2016} is used such that total running times, including training, are comparable with NUTS. For \XTryM~and \isir~the global proposal is a wide Gaussian with a pool of $N = 2000$ candidates drawn at each iteration. For MALA we tune the step size in order to keep acceptance rate approximately at $0.5$. We report the average sliced TV distance and ESS in Figure~\ref{fig:res_100d} (see \Cref{subsec:supp:metrics} for metrics definition). In most cases, \FlXTryM~is the most reliable algorithm. The only exception is at very high dimension for the banana where NUTS performs the best: in this case, tuning the flow to learn tails in high-dimension faithfully was costly such that we proceeded to an early stopping to maintain comparability with the baseline. Remarkably, \FlXTryM\ compensates significantly for the imperfect flow training, improving over adaptive-\isir, but NUTS eventually performs better. Conversely, for the funnel, most of the improvement comes from well-trained proposal flow, leading to similar behaviors of adaptive \isir\ and \FlXTryM, while both algorithms clearly outperforms NUTS in terms of metrics.


%\begin{figure}%[h]
%\centering
%\begin{subfigure}{0.49\textwidth}
%    \includegraphics[width=1\textwidth]{figures/flow_funnel_samples_2_dim_dim_2_var_2_N_3_mala_0.pdf}
%    \caption{\FlXTryM\ samples with and without rejuvenation steps}
%    \label{fig:samples_2d_funnel}
%\end{subfigure}
%\begin{subfigure}{0.49\textwidth}
%    \includegraphics[width=1\textwidth]{figures/flow_dim_2_density_var_2_N_3_mala_0.pdf}
%    \caption{$1$st coordinate marginal density KDE}
%    \label{fig:density_estimates_2d_funnel}
%\end{subfigure}
%\caption{$2$-dimensional Funnel distribution results}
%\label{fig:funnel_2d_flex}
%\end{figure}

\begin{figure}%[h]
\centering
\begin{subfigure}{0.56\textwidth}
    \includegraphics[width=1\textwidth]{figures/banana_visualize_d_100.png}
    \caption{$d = 100$, $2000$ samples projection}
    \label{fig:samples_100d_banana}
\end{subfigure}
\begin{subfigure}{0.42\textwidth}
    \includegraphics[width=1\textwidth]{figures/banana_ess_tv_study_new.png}
    \caption{Banana-shape distribution}
    \label{fig:metrics_banana}
\end{subfigure}
\begin{subfigure}{0.56\textwidth}
    \includegraphics[width=1\textwidth]{figures/funnel_visualize_d_100.png}
    \caption{$d = 100$, $1000$ samples projection}
    \label{fig:samples_100d_funnel}
\end{subfigure}
\begin{subfigure}{0.42\textwidth}
    \includegraphics[width=1\textwidth]{figures/funnel_ess_tv_study_new.png}
    \caption{Neal's funnel}
    \label{fig:metrics_funnel}
\end{subfigure}
\caption{Anisotropic Funnel and Banana-shape distributions -- (a) and (b) visualize samples projected onto the first 2 coordinates of tested algorithms (blue) versus true samples obtained by reparametrization (orange). (c) and (d) compare Sliced Total Variation and Effective Sample Size as a function of dimension. \isir\ is removed from (b) as corresponding metrics for $d > 20$ are significantly worse.}
\label{fig:res_100d}
\vspace{-5mm}
\end{figure}


%We use the HMC-based NUTS sampler~\citep{hoffman2014no} to generate reference samples and compute STV, ESS, and EMD for samples obtained from a single run of MALA, \XTryM\, and \FlXTryM. The numerical results for the asymmetric banana distribution are shown in \Cref{fig:asym_banana_metrics} and for the funnel distribution in \Cref{fig:funnel_metrics}. We clearly see the advantages of \XTryM\ over MALA in approximation quality (see also \Cref{fig:half_banana_proj}), while \FlXTryM\ provides a dramatic improvement in sampling efficiency.

\vspace{-4mm}
\subsection{Sampling from GANs as Energy-based models (EBMs)}
\vspace{-3mm}
Generative adversarial networks (GANs \cite{10.5555/2969033.2969125}) are a class of generative models defined by a pair of a generator network $G$ and a discriminator network $D$. The generator $G$ takes a latent variable $z$ from a prior density $p_0(z)$, $z \in \rset^d$, and generates an observation $G(z) \in \rset^{\dim}$ in the observation space. The discriminator takes a sample in the observation space and aims to discriminate between true examples and false examples produced by the generator. Recently, it has been advocated to consider GANs as Energy-Based Models (EBMs)~\cite{Turner2019,Che2020}.
Following~\cite{Che2020}, we consider the EBM model induced by the GAN in latent space.
% , in contrast to~\cite{Turner2019}, which operates in observational space.
Recall that an EBM is defined by a Boltzmann distribution $p(z) = \rme^{-E(z)}/\normconst$, $z \in \rset^d$, where $E(z)$ is the energy function and $\normconst$ is the normalizing constant. Note that Wasserstein GANs also allow for an energy-based interpretation (see~\cite{Che2020}), although the interpretation of the discriminator in this case is different. The energy function is given by
\begin{equation}
\label{eq:energy_funs_GANS}
\textstyle{E_{JS}(z)= -\log p_0(z) - \logit\bigl(D(G(z))\bigr)\eqsp, \quad E_{W}(z) = -\log p_0(z) - D(G(z)\bigr), \quad z \in \rset^d}\eqsp,
\end{equation}
for the vanilla Jensen-Shannon and Wasserstein GANs, respectively. Here $\logit(y),\, y \in (0,1)$ is the inverse of the sigmoid function and $p_0(z) = \mathcal{N}(0,\Id_{d})$.
% In ia advocated in~\cite{Che2020} that sampling from the models \eqref{eq:energy_funs_GANS} yields significant improvements compared to the traditional generator-only sampling. In most EBMs, samples from $p(z)$ are generated by an MCMC algorithm, either using Unadjusted Langevin Dynamics (ULA) or standard MCMC algorithms such as MALA or HMC; see~\cite{xie2018cooperative,nijkamp2020anatomy,song2021train} and references therein. We advocate the use of the \XTryM\ algorithm instead.
\vspace{-3mm}
\paragraph{MNIST results.}
We consider a simple Jensen-Shannon GAN model trained on the MNIST dataset with latent space dimension $d = 2$. We compare samples obtained by \isir, MALA, and \XTryM\ from the energy-based model associated with $E_{JS}(z)$, see \eqref{eq:energy_funs_GANS}. We use a wide normal distribution as the global proposal for \isir\ and \XTryM, and pools of candidates at each iteration $N = 10$. The step-size of MALA is tuned to keep an acceptance rate $\sim 0.5$. We visualize chains of $100$ steps in the latent space obtained with each method in \Cref{fig:mnist_energy_plots_js}. Note that the poor agreement between the proposal and the landscape makes it difficult for \isir\ to accept from the proposal and for MALA to explore many modes of the latent distribution, as shown in \Cref{fig:mnist_energy_plots_js}. \XTryM\ combines effectively global and local moves, encouraging better diversity associated with a better mixing time. The images corresponding to the sampled latent space locations are displayed in \Cref{fig:mnist_images_visualize} and reflect the diversity issue of MALA and $\isir$. Further details and experiments are provided in \Cref{supp:sec:MNIST}, including similar results for WGAN-GP \cite{gulrajani:2017:wgan} and the associated EBM $E_{W}(z)$.
\vspace{-3mm}

\begin{figure}%[h]
\centering
\begin{subfigure}{0.8\textwidth}
\captionsetup{justification=centering}
\includegraphics[width=1.0\textwidth]{figures/MNIST/energy_landscape_2d_gan_mnist.pdf}
\end{subfigure}
\vspace{-2mm}
\caption{MNIST energy landscape and single chain latent samples visualizations.}
\label{fig:mnist_energy_plots_js}
\vspace{-5mm}
\end{figure}

\paragraph{Cifar-$10$ results.}
% We consider the problem of sampling from the energy-based models, defined by the energy functions $E_{JS}(z)$ and $E_{W}(z)$ from \eqref{eq:energy_funs_GANS}.
We consider two popular architectures trained on Cifar-10, DC-GAN~\cite{radford2016unsupervised} and SN-GAN~\cite{miyato2018spectral}. In both cases the dimension of the latent space equals $d = 128$. Together with the non-trivial geometry of the corresponding energy landscapes, the large dimension makes sampling with NUTS unfeasible in terms of computational time. We perform sampling from mentioned GANs as energy-based models using \isir, MALA, \XTryM, and \FlXTryM. In \isir\ and \XTryM\ we use the prior $p_{0}(z)$ as a global proposal with a pool of $N=10$ candidates. For \FlXTryM\, we perform training and sampling simultaneously. Implementation details are provided in \Cref{supp:sec:cifar}. To evaluate sampling quality, we report the values of the energy function $E(z)$, averaged over $500$ independent runs of each sampler. {We also visualize the inception score (IS) dynamics calculated over $10000$ independent trajectories}. We present the results in \Cref{fig:cifar_10_pictures} together with the images produced by each sampler. Note that \XTryM\ and \FlXTryM\ reach low level of energies faster than other methods, {and reach high IS samples in a limited number of iterations}. Visualizations indicate that MALA is unlikely to escape the mode of the distribution $p(z)$ it started from, while \isir\ and \XTryM/\FlXTryM\ better explores the target support. However, global move appear to become more rare after some number of iterations for \XTryM/\FlXTryM, which then exploit a particular mode with MALA steps. We here hit the following limitation: $\isir$ remains at relatively high-energies, failing to explore well modes basins but still accepting global moves, while \XTryM/\FlXTryM\ explores well modes basins but eventually remains trapped. We predict that improving further the quality of the \FlXTryM\ proposal by scaling the normalizing flow architecture would allow for more global moves.See \Cref{supp:sec:cifar} for additional experiments (including ones with SN-GAN), {FID dynamics}, and visualizations.



\begin{figure}%[h]
\centering
\begin{subfigure}{0.29\textwidth}
\includegraphics[width=1\textwidth]{figures//MNIST/samples_isir_2d_mnist.pdf}
\caption{\isir\ samples}
\label{fig:samples_mnist_2d_ex2mcmc}
\end{subfigure}
\hspace{4mm}
\begin{subfigure}{0.29\textwidth}
\includegraphics[width=1\textwidth]{figures//MNIST/samples_mala_2d_mnist.pdf}
\caption{MALA samples}
\label{fig:samples_mnist_2d_ex2mcmc}
\end{subfigure}
\hspace{4mm}
\begin{subfigure}{0.29\textwidth}
\includegraphics[width=1\textwidth]{figures//MNIST/samples_ex2mcmc_2d_mnist.pdf}
\caption{\XTryM\ samples}
\label{fig:samples_mnist_2d_ex2mcmc}
\end{subfigure}
\caption{MNIST samples visualization. -- Single chains run, sequential steps.}
\label{fig:mnist_images_visualize}
\vspace{-5mm}
\end{figure}

\begin{figure}%[h]
\centering
\begin{subfigure}{0.3\textwidth}
\captionsetup{justification=centering}
\includegraphics[width=1.0\textwidth]{figures/energy_dcgan.png}
\caption{Energy decay for $100$ iterations}
\label{fig:energy_dc_gan_vis}
\end{subfigure}
\begin{subfigure}{0.25\textwidth}
\captionsetup{justification=centering}
\includegraphics[width=1.0\textwidth]{figures/is_dcgan.pdf}
\caption{IS dynamics, $1000$ iterations}
\label{fig:energy_dc_gan_vis}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
\includegraphics[width=1\textwidth]{figures/samples_ex2.png}
\caption{\XTryM\ samples}
\label{fig:samples_cifar_iters}
\end{subfigure}

\begin{subfigure}{0.48\textwidth}
\captionsetup{justification=centering}
\includegraphics[width=1.0\textwidth]{figures/samples_mala.png}
\caption{MALA samples}
\label{fig:mala_cifar_10_vis}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\captionsetup{justification=centering}
\includegraphics[width=1.0\textwidth]{figures/samples_isir.png}
\caption{\isir\ samples}
\label{fig:isir_cifar_10_vis}
\end{subfigure}
\caption{Cifar-$10$ energy and sampling results with DC-GAN architecture. Along the horizonthal lines we visualize each $10$th sample from a single trajectory.}
\label{fig:cifar_10_pictures}
\vspace{-5mm}
\end{figure}


==> Local - (learned) Global Mixed Kernels/sec_related.tex <==
% \isir\ was proposed by~\cite{andrieu2010particle} and further developed in~\citep{andrieu2018uniform}; see also~\citep{lee2010utility,lee2011auxiliary}.

%\isir\ has connections to particle Gibbs methods, as highlighted in \cite{andrieu2018uniform}. The main difference is that the proposal distribution for the latter is defined on the ''path space'' used in sequential Monte Carlo methods; see also~\citep{doucet2015efficient}. Using this analogy, the rejuvenation kernel of \XTryM\ plays a role similar to that of the backward sampling kernel in particle Gibbs with backward sampling (PGBS; \cite{lindsten2013backward}). \marylou {Maybe this should be developed?} \eric{only partially true}

%\XTryM\ algorithm can also be considered as a summarized version of the Gibbs sampler proposed in~\citep{tjelmeland2004using}. \marylou{Is this the case for \isir~ or just \XTryM?}


% Related works focusing on adaptive schemes
\vspace{-3mm}
The possibility to parametrize very flexible probabilistic models with neural networks thanks to deep learning has rekindled interest in adapting MCMC kernels; see \eg\  \cite{song2017nice,Hoffman2019,albergo:2019,Nicoli2020,Hackett2021}. While significant performance gain were found in problems of moderate dimensions, these learning-based methods were found to suffer from increasing dimensions as fitting models accurately becomes more difficult \cite{DelDebbio2021,Mahmoud2022}. Similarly to \FlXTryM, a few work proposed adaptive algorithms that alternates between global and local MCMC moves to ensure ergodicity without requiring a perfect learning of the proposal\cite{Pompe2020,Gabrie2021}. {More precisely}, \cite{Pompe2020} focused on multimodal distributions and analysed a mode jumping algorithm using proposals parametrized as mixture of simple distributions. While \cite{Gabrie2021}, closer to this work, introduced a combination of a local and a global sampler {leveraging normalizing flows} with a more classical choice for the global sampler: independent Metropolis-Hasting (IMH) instead of \isir. {The present work builds on these previous propositions of combinations of local and global sampler by clarifying the reasons of their effectiveness through entirely novel detailed mathematical and empirical analyses. We chose to focus on $\isir$ with an adaptive proposal as the global sampler since (i) the learning component allows to tackle high-dimensional targets, (ii) theoretical guarantees can be obtained for \isir~whereas IMH is more difficult to analyze, (iii) IMH and \isir~(as a multiple-try MCMC) are expected to have similar performances for comparable computational budget \cite{bedard2012scaling} but IMH is sequential where $\isir$ can be parallelized by increasing the number $N$ of proposals per iteration.}


Another line of work exploits both normalizing flows and common local MCMC kernels for sampling \cite{Parno2018,Hoffman2019,Noe2019,Zhang2022}, {yet following the different paradigm of using the flow as a reparametrization map, a method sometimes referred to as neural transport:} the flow $T$ is trained to transport a simple distribution $\proposalbase$ near $\target$, which is equivalent to bringing $\pushforward[T^{-1}][\target]$ (the pushforward of the original target distribution $\target$ by the inverse flow $T^{-1}$) close to $\proposalbase$. If $\proposalbase$ is simple enough to be efficiently sampled by local samplers, the hope is that local samplers can also obtain high-quality samples of $\pushforward[T^{-1}][\target]$ -- samples which can be transported back through $T$ to obtain samples of $\target$. This method {attempts} to reparametrize the space to disentangle problematic geometries for local kernels. Yet, it is unclear what will happen in the tails of the distribution for which the flow is likely poorly learned. Furthermore, in order to derive an ergodicity theory for these transported samplers, \cite{Parno2018} necessitated substantial constraints on maps (see section 2.2.2.).  



==> algo_ex2.tex <==
\begin{algorithm2e}[t!]
    \SetKwInOut{In}{Input}
    \SetKwInOut{Out}{Output}
    \caption{Single stage of \XTryM\ algorithm with independent proposals}
    \label{alg:X-Try-MCMC}
    \SetKwFunction{KwPrint}{print}
    \SetKwProg{Fn}{Procedure \ }{:}{end}
    \SetKwFunction{X-Try}{X-Try SIR}
    \SetKwProg{myalg}{Algorithm}{}{}
    \Fn{\XTryM\ $(Y_k,\proposal,\rejukernel)$}{
    \In{Previous state $Y_{k}$; proposal distribution $\proposal$; rejuvenation kernel $\rejukernel$;}
    \Out{New sample $Y_{k+1}$; pool of proposals $\chunku{X}{2}{N}_{k+1} \sim \proposal$;}
    $Z_{k+1}\eqsp, \chunku{X}{2}{N}_{k+1} = \isir(Y_{k},\proposal)$; \\
    Draw $Y_{k+1} \sim \rejukernel(Z_{k+1},\cdot)$. \\
    %For $i \in \range{N}$, compute the normalized weights $\unormweight_i[k+1]= \weightfunc(X^{i}[k+1])$. \\
    %Compute $\NormFactor[k+1] = \sum_{i=1}^N \unormweight_i[k+1]$. \\
    %\For{$i \in \range{N}$}{
    %    compute the normalized weights $\normweight_{i,k+1}= \weightfunc(X^{i}_{k+1})/\sum_{\ell=1}^N\weightfunc(X^{\ell}_{k+1})$; \\
    %    }
    %Draw the proposal index $I_{k+1} \sim \mathrm{Cat}(\normweight_{1,k+1},\dots,\normweight_{N,k+1})$; \\
    %Draw  $Y_{k+1}\sim \rejukernel(X^{I_{k+1}}_{k+1},\cdot)$. \\
    }
    \vspace{-3pt}
\end{algorithm2e} 
\vspace{-3mm}

==> algo_isir.tex <==
\begin{algorithm2e}[t!]
    \SetKwInOut{In}{Input}
    \SetKwInOut{Out}{Output}
    \caption{Single stage of \isir\ algorithm with independent proposals}
    \label{alg:i-sir-MCMC}
    \SetKwFunction{KwPrint}{print}
    \SetKwProg{Fn}{Procedure \ }{:}{end}
    \SetKwFunction{X-Try}{iterated SIR}
    \SetKwProg{myalg}{Algorithm}{}{}
    \Fn{\isir\ $(Y_k,\proposal)$}{
    \In{Previous state $Y_{k}$; proposal distribution $\proposal$;}
    \Out{New state $Y_{k+1}$; pool of proposals $\chunku{X}{2}{N}_{k+1} \sim \proposal$;}
    Set $X^1_{k+1}= Y_{k}$, draw $\chunku{X}{2}{N}_{k+1} \sim \proposal$; 
    \For{$i \in \range{N}$}{
        compute the normalized weights $\normweight_{i,k+1}= \weightfunc(X^{i}_{k+1})/\sum_{\ell=1}^N\weightfunc(X^{\ell}_{k+1})$; \\
        }
    Draw the proposal index $I_{k+1} \sim \mathrm{Cat}(\normweight_{1,k+1},\dots,\normweight_{N,k+1})$; \\
    Set $Y_{k+1} := X^{I_{k+1}}_{k+1}$. \\
    }
\vspace{-3pt}
\end{algorithm2e} 


==> conclusion.tex <==
\vspace{-3mm}
%\marylou{Tuning down the allegation of novelty - the combination is relatively simple}
The present paper examines the benefits of combining local and global samplers. From a theoretical point of view, we show that global samplers are more robust when coupled with local samplers. Namely, a $V$-geometric ergodicity is obtained for the $\XTryM$ kernel under minimal assumptions. Meanwhile, the global samplers drives exploration when properly adjusted. Therefore, we also describe the adaptive version $\FlXTryM$ of the strategy involving the learning of a global proposal parametrized by a normalizing flow. We also check for the learning convergence along the adaptive MCMC run. Finally, a series of numerical experiments confirms the superiority of the strategy, including the high-dimensional examples.
While the startegy was described and analyzed for the \isir~global kernel, we note that it would be possible to extend the theory to other independent global samplers. We expect that the benefit of the combination would remain. Further studies of \FlXTryM, in particular the derivation of its mixing rate, is an interesting direction for future work.
% We propose a new MCMC algorithm, \XTryM, which allows to improve over the competitors due to the efficiency both at exploration and exploitation steps. We analyze its theoretical properties and suggest an adaptive version of the algorithm, \FlXTryM, based on normalizing flows. It allows to overcome the issues of MTM and \isir\ algorithms, which are caused by low acceptance rate when sampling from high dimensional distributions. Further studies of \FlXTryM, in particular its mixing rate, is an interesting direction for the future work

==> sec_adaptive.tex <==
%% Outline
% Performance of IS based sampling controlled by \weightfunc = ...
% Natural to try to improve the proposal to match the target, tradition of adaptive MCMC.
% Describe the concept
% Even more so with deep generative models, flexibility could make us hope to closely match target, in particular normalizing flows.
%
\vspace{-2mm}
The performance of proposal-based samplers depends on the distribution of importance weights which is related to the similarity of the proposal and target distributions\footnote{more specifically, it depends on the the quantities appearing in \Cref{assum:independent-proposal}, namely, the maximum of the importance weight on a level set of the drift function for the local kernel $\rejukernel$ and the variance of the importance weights under the proposal}.
Therefore, yet another strategy to improve sampling performance is to select the proposal distribution $\proposal$ from a family of parameterized distributions $\left\{\proposal_{\theta}\right\}$ and fit the parameter $\theta \in \Theta = \rset^q$ to the target $\target$, for example, by minimizing a Kullback-Leibler divergence (KL) \cite{Parno2018, albergo:2019, Naesseth2020} or matching moments \cite{Pompe2020}. In \emph{adaptive MCMCs}, parameter adaptation is performed along the MCMC run  \cite{andrieu2006ergodicity,andrieu2008tutorial,roberts2009examples}. In this section we propose an adaptive version of \XTryM, which we call \FlXTryM.


\textbf{Normalizing flow proposal.}
A flexible way to parameterize proposal distributions is to combine a tractable distribution $\proposalbase$ with an invertible parameterized transformation. Let $T: \Xset \mapsto \Xset$ be a $\rmc^1$ diffeomorphism. We denote by $\pushforward[T][\proposalbase]$ the push-forward of $\proposalbase$ under $T$, that is, the distribution of $X=T(Z)$ with $Z\sim\proposalbase$. Assuming that $\proposalbase$ has a p.d.f. (also denoted $\pdfproposalbase$), the corresponding push-forward density (w.r.t. the Lebesgue measure) is given by $\pdfproposal_T(y) = \pdfproposalbase\bigl(T^{-1}(y)\bigr) \jacop{T^{-1}}(y)$, where $\jacop{T}$ denotes the Jacobian determinant of $T$. The parameterized family of diffeomorphisms $\{T_\theta\}_{\theta \in \Theta}$ defines a family of distributions $\{\pdfproposal_{T_\theta}\}_{\theta \in \Theta}$, denoted for simplicity as $\{\pdfproposal_\theta\}_{\theta \in \Theta}$.
This construction is called a \emph{normalizing flow} (NF) and a great deal of work has been devoted to ways of parameterizing invertible flows $T_{\theta}$ with neural networks; see~\citep{kobyzev2020normalizing,papamakarios2019normalizing} for reviews.

\textbf{Simultaneous learning and sampling.} {As with adaptive MCMC methods, the parameters of a NF proposal are learned for the global proposal during sampling, see also \cite{Gabrie2021}.} We work with $M$ copies of the Markov chains $\{(Y_k[j], \chunku{X_k}{1}{N}[j])\}_{k \in \nsets}$ indexed by $j \in \{1,\dots, M \}$. At each step $k \in \nsets$, each copy is sampled as in \XTryM~using the NF proposal, independently from the other copies, but conditionally to the the current value of the parameters $\theta_{k-1}$.
% , \ie\
% \begin{equation}
%     X_k^1[j]= Y_{k-1}[j] \, \text{ and } \, X_k^{\ell}[j] = T_{\theta_{k-1}}(Z_k^{\ell}[j]), \ell \in \{2,\dots,N\} \, \text{ where } \, \{ \chunku{Z}^{2:N}_k[j] \} \simiid \proposalbase.
% \end{equation}
We then adapt the parameters by taking steps of gradient descent on a convex combination of the \emph{forward} KL, $\KL{\pdftarget}{\pdfproposal_\theta} = \int_{} \pdftarget(x) \log(\pdftarget(x)/\pdfproposal_\theta(x)) \rmd x$ and the backward KL  $  \KL{\pdfproposal_\theta}{\pdftarget} = \int \pdfproposal_\theta(x) \log (\pdftarget(x)/\pdfproposal_\theta(x)) \rmd x = \int \pdfproposalbase(z) \log \weightfunc_\theta \circ T_\theta(z)  \rmd z$.
Let $\sequence{\gamma}[k][\nset]$ be a sequence of nonnegative stepsizes and $\sequence{\alpha}[k][\nset]$ be a nondecreasing sequence in $\ccint{0,1}$ with $\alpha_{\infty}= \lim_{k \to \infty} \alpha_k$.
The update rule is $\theta_k= \theta_{k-1} + \gamma_k M^{-1} \sum_{j=1}^M  H(\theta_{k-1},\chunku{X_k}{1}{N}[j],\chunku{Z_k}{2}{N}[j])$ where  $H(\theta,\chunku{x}{1}{N},\chunku{z}{2}{N})= \alpha_k H^{f}(\theta,\chunku{x}{1}{N})+
(1-\alpha_k) H^b(\theta,\chunku{z}{2}{N})$ with
\begin{align}
\label{eq:fwdKL}
H^{f}(\theta,\chunku{x}{1}{N}) &=  \sum\nolimits_{\ell=1}^N \frac{\weightfunc_{\theta}(x^{\ell})}{\sum\nolimits_{i=1}^N \weightfunc_{\theta}(x^i)} \nabla_{\theta} \log \pdfproposal_{\theta}(x^{\ell})  \eqsp, \quad \weightfunc_\theta(x)= \pdftarget(x)/ \pdfproposal_\theta(x)\eqsp, \\
\label{eq:bwdKL}
H^b(\theta,\chunku{z}{2}{N})&= 
 - \frac{1}{N-1} \sum\nolimits_{\ell=2}^N \{ \nabla_\theta \log \pdftarget \circ T_\theta(z^\ell) + \nabla_\theta \log \jacop{T_\theta} (z^{\ell}) \}\eqsp.
\end{align}
Note that we use a Rao-Blackwellized estimator of the gradient of the forward KL \eqref{eq:fwdKL} where we fully recycle all the $N$ candidates sampled at each iteration of \isir. The quality of this estimator is expected to improve along the iterations $k$ of the algorithm as the variance of importance weights decreases as the proposal improves. Note also that using only gradients from the backward KL \eqref{eq:bwdKL} is prone to mode-collapse \cite{Parno2018,Noe2019,Naesseth2020,Gabrie2021}, hence the need for also using gradients from the forward KL $H^{f}(\theta,\chunku{x}{1}{N})$, which requires the simultaneous sampling from $\target$. {See also \Cref{app:subsec:mixture-highd} for further discussions.}
{The \FlXTryM\ algorithm is summarized in \Cref{alg:NF-X-Try-MCMC}.} 

Since the parameters of the Markov kernel $\theta_{k}$ are updated using samples $\chunku{X_k}{1}{N}$ from the chain, $\dsequence{Y}{\chunku{X}{1}{N}}[k][\nset]$ is no longer Markovian. This type of problems has been considered in \cite{metivier1987theoremes,benveniste1990adaptive,gu1998stochastic,andrieu2005stability} and to prove convergence of the strategy we need to strengthen assumptions compared to the previous section.
\begin{assumption}
\label{assum:condition-gradient}
There exists a function $W: \Xset \to \rset_+$ such that $\proposalbase(W^2)= \int W^2(z) \proposalbase(\rmd z) < \infty$, and a constant $L < \infty$ such that, for all $\theta, \theta' \in \Theta$ and $z \in \Xset$, $\Vert \nabla_\theta \log \target \circ T_\theta(z) - \nabla_\theta \log \target \circ T_{\theta'}(z)\Vert \leq L \| \theta - \theta' \| W(z)$ and $ \Vert \nabla_\theta \log \jacop{T_\theta} (z) - \nabla_\theta \log \jacop{T_{\theta'}} (z) \Vert \leq L \norm{\theta - \theta'} W(z)$.
\end{assumption}
\begin{assumption}
\label{assum:independent-proposal-strengthen}
(i) For all $d \geq d_{\rejukernel}$, $\weightfunc_{\infty, d}= \sup_{\theta \in \Theta} \sup_{x\in\msv_d} \weightfunc_\theta(x) / \proposal_\theta(\weightfunc_\theta) < \infty$ and (ii) $\sup_{\theta \in \Theta} \PVar_{\proposalbase}(\weightfunc_\theta \circ T_\theta)/ \{ \proposal_\theta(\weightfunc_\theta) \}^2 < \infty$.
\end{assumption}
\Cref{assum:condition-gradient} is a continuity condition on the NF push-forward density \wrt~its parameters $\theta$. \Cref{assum:independent-proposal-strengthen} implies that the Markov kernel $\XtryK[N,\theta] = \MKisir[N,\theta] \rejukernel$ satisfies a drift and minorization condition uniform in $\theta$.
\begin{theorem}[simplified]
\label{thm:KL-simplified}
Assume \Cref{assum:rejuvenation-kernel}-\Cref{assum:condition-gradient}-\Cref{assum:independent-proposal-strengthen} and that $\sum_{k=0}^\infty \gamma_k = \infty$, $\sum_{k=0}^{\infty} \gamma_k^2 < \infty$ and $\lim_{k \to \infty} \alpha_k= \alpha_\infty$. Then, w.p. 1, the sequence $\sequence{\theta}[k][\nset]$ converges to the set
$\{\theta \in \Theta,  0 = \alpha_\infty \nabla \KL{\target}{\proposal_\theta} + (1-\alpha_\infty) \nabla \KL{\proposal_\theta}{\target} \}$.
\end{theorem}
\Cref{thm:KL-simplified} proves the convergence of the learning of parameters $\theta$ to a stationary point of the loss. The proof is postponed to \Cref{sec:thm:KL-simplified}.
Note that once the proposal learning has converged, $\FlXTryM$ boils back to $\XTryM$ with a fixed learned proposal. 
Our experiments show that
adaptivity can significantly speed up mixing for \isir, especially for distributions with complex geometries and that the addition of a rejuvenation kernel
further improves samples quality.

{
\input{algo_flex}
}

==> sec_intro.tex <==

% In this paper,
We consider the setting where a target distribution $\target$ on a measurable space $(\Xset,\Xsigma)$ is known up to a normalizing constant and one tries to estimate the expectations of some function $f : \Xset \to \rset$ with respect to $\target$. Examples include the extraction of Bayesian statistics from posterior distributions derived from observations as well as the computation of observables of a physical system $x \in \Xset$ under the Boltzmann distribution with non-normalized density $\pdftarget(x)= \rme^{- \beta U(x)}$ for the energy function $U$ at the inverse temperature $\beta$.


A common strategy to tackle this estimation is to resort to Markov chain Monte Carlo algorithms (MCMCs). The MCMC approach aims to simulate a realization of a time-homogeneous Markov chain $\sequence{Y}[n][\nset]$, such that the distribution of the $n$-th iterate $Y_n$ with $n \to \infty$ is arbitrarily close to $\target$, regardless of the initial distribution of $Y_0$. In particular, the Metropolis-Hastings kernel (MH) is the cornerstone of MCMC simulations, with a number of successful variants following the process of a \emph{proposal} step followed by an \emph{accept/reject} step (see e.g. \cite{robert:2015:mh}). In large dimensions, proposal distributions are typically chosen to generate local moves that depend on the last state of the chain in order to guarantee an admissible acceptance rate. However, local samplers suffer from long mixing times as
% , especially in large dimension. 
exploration is inherently slow, and mode switching, when there is more than one, can be extremely infrequent.

On the other hand, independent proposals are able to generate more global updates, but they are difficult to design. Developments in deep generative modelling, in particular versatile autoregressive and normalising flows \cite{kingma:2016:aif,huang:2018:neural_aif,dinh:2016,papamakarios2019normalizing}, spurred efforts to use learned probabilistic models to improve the exploration ability of MCMC kernels. Among a rapidly growing body of work, references include \cite{Hoffman2019, albergo:2019, Nicoli2020, Gabrie2021, Hackett2021}. While these works show that global moves in a number of practical problems can be successfully informed by machine learning models, it remains the case that the acceptance rate of independent proposals decreases dramatically with dimensions -- except in the unrealistic case that they perfectly reproduce the target. This is a well-known problem in the MCMC literature \cite{Bengtsson:2008:Curse,Bickel:2008:obstacle,agapiou2017importance}, and it was recently noted that deep learning-based suggestions are no exception in works focusing on physical systems \cite{DelDebbio2021,Mahmoud2022}.

In this paper we focus on the benefits of combining local and global samplers. Intuitively, local steps interleaved between global updates from an independent proposal (learned or not) increase accuracy by allowing accurate sampling in tails that are not usually well handled by the independent proposal. Also, mixing time is usually improved by the local-global combination, which prevents long chains of consecutive rejections. Here we focus on a global kernel of type iterative-sampling importance resampling (\isir) \citep{tjelmeland2004using,andrieu2010particle,andrieu2018uniform}. This kernel uses multiple proposals in each iteration to take full advantage of modern parallel computing architectures. For local samplers, we consider common techniques such as Metropolis Adjusted Langevin (MALA) and Hamiltonian Monte Carlo (HMC). We call this combination strategy Explore-Exploit MCMC (\XTryM) in the following.

\vspace{-2mm}
\paragraph{Contributions} The main contributions of the paper are as follows:
\begin{itemize}[leftmargin=*,noitemsep]
\vspace{-2mm}
\item We provide theoretical bounds on the accuracy and convergence speed of \XTryM\ strategies. In particular, we prove $V$-uniform geometric convergence of \XTryM\ under assumptions much milder than those required to prove uniform geometric ergodicity of the global sampler \isir~alone. %We also evaluate the relative improvement of the mixing time when local and global moves are used synergetically.
\item We {provide convergence guarantees for} an adaptive version of the strategy, called \FlXTryM, which involves learning an efficient proposal while  sampling, as in adaptive MCMC.
\item We perform a numerical evaluation of \XTryM\ and \FlXTryM\ for various sampling problems, including sampling GANs as energy-based models. The results clearly show the advantages of the {combined} approaches compared to purely local or purely global MCMC methods.
\end{itemize}
\vspace{-3mm}
\paragraph{Notations} Denote $\nsets = \nset \setminus \{0\}$. For a measurable function $f: \Xset \mapsto \rset$, we define $\supnorm{f} = \sup_{x \in \Xset}|f(x)|$ and $\target(f) := \int_{\Xset} f(x) \target(\rmd x)$. For a function $V: \Xset \mapsto [1, \infty)$ we introduce the $V$-\emph{norm} of two probability measures $\xi$ and $\xi'$ on $(\Xset,\Xsigma)$, $\Vnorm{\xi - \xi'} \eqdef \sup_{|f(x)| \leq V(x)} |\xi(f) - \xi'(f)|$. If $V\equiv 1$, $\Vnorm [1]{\cdot}$ is equal to the total variation distance (denoted $\tvnorm{\cdot}$).




==> sec_numerics.tex <==
\vspace{-3mm}
\subsection{Synthetic examples}
\label{subsec:toy_examples}
\vspace{-3mm}
\paragraph{Multimodal distributions.}
Let us start with a toy example highlighting differences between purely global \isir, purely local MALA and \XTryM\ combining both. We consider sampling from a mixture of $3$ equally weighted Gaussians in dimension $d = 2$. In \Cref{fig:gaus_example_2d}, we compare single chains produced by each algorithms. The global proposal is a wide Gaussian, with pools of $N=3$ candidate. The MALA stepsize is chosen to reach a target acceptance rate of $\sim 0.67$. This simple experiment illustrates the drawbacks of both approaches: \isir\ samples reach all the modes of the target, but the chains often get stuck for several steps hindering variability. MALA allows for better local exploration of each particular mode, yet it fails to cover all the target support. Meanwhile, \XTryM\ retains the benefits of both methods, combining the \isir-based global exploration with MALA-based local exploration.
% \begin{figure}%[h]
% \centering
% \begin{subfigure}{0.8\textwidth}
% \centering
% % \captionsetup{justification=centering}
% \includegraphics[width=1.0\textwidth]{NeurIPS/figures/toy_samples_2d_gaus_tight.pdf}
% \end{subfigure}
% \caption{Single chain mixing visualization. -- Blue color levels represent the target 2d density. Random chain initialization is noted in black, $100$ steps are plotted per sampler: the size of each red dot corresponds to the number of consecutive steps the walkers remains at a given location. For MALA, we generate $300$ samples and choose each $3$-rd one for comparability. Note that the variance of the global proposal (dotted countour lines) should be relatively large to cover well all the modes. The step size of MALA also can not be increased much to keep reasonable acceptance ratio.}
% \label{fig:gaus_example_2d}
% \vspace{-3mm}
% \end{figure}

\vspace{-1mm}
{In larger dimensions, an adaptive proposal is necessary. In \Cref{app:subsec:mixture-highd} we show that \FlXTryM~can mix between modes of a $50d$ Gaussian mixture, provided that the rough location of all the modes is known and used to initialize walkers. We also stress the robustness of the on-the-fly training exploiting running MCMC chains to evaluate the forward KL term of the loss.}

To illustrate further the performance of the {combined kernel}, we keep the $2d$ target mixture model yet assigning the uneven weights $(2/3, 1/6, 1/6)$ to the $3$ modes. We start $M$ chains drawing from the initial distribution $\xi \sim \mathcal{N}(0,4\Id_d)$ and use the same hyper-parameters as above. In \Cref{fig:mog_burnin} we provide a simple illustration to the statement \eqref{eq:tv_dist_isir} and \Cref{theo:main-geometric-ergodicity}, namely we compare  the target density to the instantaneous distributions for each sampler propagating $\xi$ during burn-in steps. As MALA does not mix easily between modes, the different statistical weights of the different modes can hardly be rendered in few iterations and KL and TV distances stalls after a few iterations. \isir\ can visit the different modes, yet it does not necessarily move at each step which slows down its covering of the modes full support, which again shows in the speed of decrease of the TV and KL. Overcoming both of these shortcomings, \XTryM\ instantaneous density comes much closer to the target. Finally, \Cref{fig:mog_single_chain} evaluates the same metrics yet for the density estimate obtained with single chain samples after burn-in. Results demonstrate once again the superiority of \XTryM.
Further details on these experiments can be found in \Cref{supp:subsec:mixtures}.


% To compare the quality of the methods, we perform the following procedure
% \begin{itemize}[leftmargin=*,nosep]
%     \item starting with the initial distribution $\mathcal{N}(0,4\Id)$, we generate the trajectory $(X_1,\ldots,X_n)$ for different values of $n \in [25,800]$ for each of the compared methods (\isir\, MALA, \XTryM\ ). Sampler hyperparameters are the same as above, and the burn-in period equals $50$;
%     \item We perform the kernel density estimate (KDE) $\widehat{p}_{n}$ based on the observations $(X_1,\ldots,X_n)$, and compute the total variation distance between $\widehat{p}_{n}$ and the target density $p_{\beta}$, and the forward $\KL{\widehat{p}_{n}}{p_{\beta}}$. Then we average the results over $100$ independent runs of each sampler.
% \end{itemize}
% The results for each sampler are reported in \Cref{fig:kl_loss} and \Cref{fig:tv_loss}. We also provide a simple illustration to the statements of \eqref{eq:tv_dist_isir} and \Cref{theo:main-geometric-ergodicity}. Starting with the initial distribution $\xi \sim \mathcal{N}(0,4\Id)$, we sample $500$ independent chains of length $50$ for each of the compared methods. Upon these $500$ observations we build a KDE $\widehat{p}_{n}$ for the density corresponding to the distribution of $\xi \MKQ^{n}$ for different $n \in \{5,\ldots,50\}$ and $\MKQ$ corresponding to \isir\, MALA, or \XTryM\ . Then we compute the total variation distance between $\widehat{p}_{n}$ and the target density $p_{\beta}$. Corresponding plots are shown in \Cref{fig:tv_loss_parallel} and \Cref{fig:gaus_2d_loss_plots}. Note that \XTryM\ significantly outperforms the results of both MALA and \isir\ . Indeed, the inhomogeneous mixture model is complicated target for the Langevin-based methods. The MALA -generated trajectories tend to stay in one mode of the mixture \eqref{eq:gaus_mixture}, which decreases the reliability of the estimates, and requires to generate long trajectories even in case $d = 2$. At the same time, for \isir\ -type methods without local exploration moves it is hard to balance the time spent in one of the distribution modes.
% \vspace{-3mm}

\begin{figure}%[h]
\begin{minipage}{0.69\textwidth}
\centering
{\includegraphics[width=1.0\textwidth]{figures/toy_samples_2d_gaus_new.png}\label{fig:gaus_example_2d}}
\end{minipage}
\begin{minipage}{0.3\textwidth}
\centering
\begin{subfigure}{1.0\textwidth}
    \centering
    \captionsetup{justification=centering}
    \includegraphics[width=0.6\textwidth]{figures/3_gaussians/3_gauss_forward_KL_parallel.png}
    \vspace{-3mm}
    \caption{}
%     \caption{Forward KL between the parallel iterates}
%     \label{fig:tv_loss_parallel}
% \end{subfigure}
% \begin{subfigure}{0.24\textwidth}
    % \includegraphics[width=0.49\textwidth]{figures/3_gaussians/3_gauss_TV_parallel.png}
    % \caption{Parallel iterates burn-in ($M=500$ chains KDE)}
    \label{fig:mog_burnin}
\end{subfigure}
\\
\vspace{-1mm}
\begin{subfigure}{1.0\textwidth}
    \centering
    \captionsetup{justification=centering}
    \includegraphics[width=0.6\textwidth]{figures/3_gaussians/3_gauss_forward_KL.png}
    \vspace{-3mm}
    \caption{}
%       \caption{Forward KL}
%     \label{fig:kl_loss}
% \end{subfigure}
% \begin{subfigure}{0.24\textwidth}
    %   \includegraphics[width=0.49\textwidth]{figures/3_gaussians/3_gauss_TV.png}
    %   \caption{Single chain efficiency ($M=100$ average)}
    \label{fig:mog_single_chain}
\end{subfigure}
\label{fig:gaus_2d_loss_plots}
\end{minipage}
\vspace{-1mm}
\caption{(a) -- Single chain mixing visualization. -- Blue color levels represent the target 2d density. Random chain initialization is noted in black, $100$ steps are plotted per sampler: the size of each red dot corresponds to the number of consecutive steps the walkers remains at a given location. %For MALA, we generate $300$ samples and choose each $3$-rd one for comparability. 
Note that the variance of the global proposal (dotted countour lines) should be relatively large to cover well all the modes. %The step size of MALA also can not be increased much to keep reasonable acceptance ratio.\\
(b - c) -- Inhomogeneous 2d Gaussian mixture. -- Quantitative analysis during burn-in of parallel chains (b, $M=500$ chains KDE) and for after burn-in for single chains statistics (c, $M=100$ average).}
\vspace{-5mm}
\end{figure}
\vspace{-4mm}
\paragraph{Distributions with complex geometry.}
Next, we turn to highly anisotropic distributions in high dimensions. Following \cite{neal:slice:2003} and \cite{haario1999banana}, we consider the \emph{funnel} and the \emph{banana-shape} distributions. We remind densities in \Cref{supp:subsec:complex-geometry} along with providing experiments details. For $d \in [10; 200]$, we run \isir, MALA, \XTryM, \FlXTryM, adaptive \isir~ (using the same proposal as \FlXTryM, but without interleaved local steps) and the versatile sampler NUTS~\cite{hoffman2014no} as a baseline. Here the parameter adaptation for $\FlXTryM$ is performed in a pre-run and parameters are frozen before sampling.
% to sample $1000$ points.
For the adaptive samplers, a simple RealNVP-based normalizing flow \cite{dinh:2016} is used such that total running times, including training, are comparable with NUTS. For \XTryM~and \isir~the global proposal is a wide Gaussian with a pool of $N = 2000$ candidates drawn at each iteration. For MALA we tune the step size in order to keep acceptance rate approximately at $0.5$. We report the average sliced TV distance and ESS in Figure~\ref{fig:res_100d} (see \Cref{subsec:supp:metrics} for metrics definition). In most cases, \FlXTryM~is the most reliable algorithm. The only exception is at very high dimension for the banana where NUTS performs the best: in this case, tuning the flow to learn tails in high-dimension faithfully was costly such that we proceeded to an early stopping to maintain comparability with the baseline. Remarkably, \FlXTryM\ compensates significantly for the imperfect flow training, improving over adaptive-\isir, but NUTS eventually performs better. Conversely, for the funnel, most of the improvement comes from well-trained proposal flow, leading to similar behaviors of adaptive \isir\ and \FlXTryM, while both algorithms clearly outperforms NUTS in terms of metrics.


%\begin{figure}%[h]
%\centering
%\begin{subfigure}{0.49\textwidth}
%    \includegraphics[width=1\textwidth]{figures/flow_funnel_samples_2_dim_dim_2_var_2_N_3_mala_0.pdf}
%    \caption{\FlXTryM\ samples with and without rejuvenation steps}
%    \label{fig:samples_2d_funnel}
%\end{subfigure}
%\begin{subfigure}{0.49\textwidth}
%    \includegraphics[width=1\textwidth]{figures/flow_dim_2_density_var_2_N_3_mala_0.pdf}
%    \caption{$1$st coordinate marginal density KDE}
%    \label{fig:density_estimates_2d_funnel}
%\end{subfigure}
%\caption{$2$-dimensional Funnel distribution results}
%\label{fig:funnel_2d_flex}
%\end{figure}

\begin{figure}%[h]
\centering
\begin{subfigure}{0.56\textwidth}
    \includegraphics[width=1\textwidth]{figures/banana_visualize_d_100.png}
    \caption{$d = 100$, $2000$ samples projection}
    \label{fig:samples_100d_banana}
\end{subfigure}
\begin{subfigure}{0.42\textwidth}
    \includegraphics[width=1\textwidth]{figures/banana_ess_tv_study_new.png}
    \caption{Banana-shape distribution}
    \label{fig:metrics_banana}
\end{subfigure}
\begin{subfigure}{0.56\textwidth}
    \includegraphics[width=1\textwidth]{figures/funnel_visualize_d_100.png}
    \caption{$d = 100$, $1000$ samples projection}
    \label{fig:samples_100d_funnel}
\end{subfigure}
\begin{subfigure}{0.42\textwidth}
    \includegraphics[width=1\textwidth]{figures/funnel_ess_tv_study_new.png}
    \caption{Neal's funnel}
    \label{fig:metrics_funnel}
\end{subfigure}
\caption{Anisotropic Funnel and Banana-shape distributions -- (a) and (b) visualize samples projected onto the first 2 coordinates of tested algorithms (blue) versus true samples obtained by reparametrization (orange). (c) and (d) compare Sliced Total Variation and Effective Sample Size as a function of dimension. \isir\ is removed from (b) as corresponding metrics for $d > 20$ are significantly worse.}
\label{fig:res_100d}
\vspace{-5mm}
\end{figure}


%We use the HMC-based NUTS sampler~\citep{hoffman2014no} to generate reference samples and compute STV, ESS, and EMD for samples obtained from a single run of MALA, \XTryM\, and \FlXTryM. The numerical results for the asymmetric banana distribution are shown in \Cref{fig:asym_banana_metrics} and for the funnel distribution in \Cref{fig:funnel_metrics}. We clearly see the advantages of \XTryM\ over MALA in approximation quality (see also \Cref{fig:half_banana_proj}), while \FlXTryM\ provides a dramatic improvement in sampling efficiency.

\vspace{-4mm}
\subsection{Sampling from GANs as Energy-based models (EBMs)}
\vspace{-3mm}
Generative adversarial networks (GANs \cite{10.5555/2969033.2969125}) are a class of generative models defined by a pair of a generator network $G$ and a discriminator network $D$. The generator $G$ takes a latent variable $z$ from a prior density $p_0(z)$, $z \in \rset^d$, and generates an observation $G(z) \in \rset^{\dim}$ in the observation space. The discriminator takes a sample in the observation space and aims to discriminate between true examples and false examples produced by the generator. Recently, it has been advocated to consider GANs as Energy-Based Models (EBMs)~\cite{Turner2019,Che2020}.
Following~\cite{Che2020}, we consider the EBM model induced by the GAN in latent space.
% , in contrast to~\cite{Turner2019}, which operates in observational space.
Recall that an EBM is defined by a Boltzmann distribution $p(z) = \rme^{-E(z)}/\normconst$, $z \in \rset^d$, where $E(z)$ is the energy function and $\normconst$ is the normalizing constant. Note that Wasserstein GANs also allow for an energy-based interpretation (see~\cite{Che2020}), although the interpretation of the discriminator in this case is different. The energy function is given by
\begin{equation}
\label{eq:energy_funs_GANS}
\textstyle{E_{JS}(z)= -\log p_0(z) - \logit\bigl(D(G(z))\bigr)\eqsp, \quad E_{W}(z) = -\log p_0(z) - D(G(z)\bigr), \quad z \in \rset^d}\eqsp,
\end{equation}
for the vanilla Jensen-Shannon and Wasserstein GANs, respectively. Here $\logit(y),\, y \in (0,1)$ is the inverse of the sigmoid function and $p_0(z) = \mathcal{N}(0,\Id_{d})$.
% In ia advocated in~\cite{Che2020} that sampling from the models \eqref{eq:energy_funs_GANS} yields significant improvements compared to the traditional generator-only sampling. In most EBMs, samples from $p(z)$ are generated by an MCMC algorithm, either using Unadjusted Langevin Dynamics (ULA) or standard MCMC algorithms such as MALA or HMC; see~\cite{xie2018cooperative,nijkamp2020anatomy,song2021train} and references therein. We advocate the use of the \XTryM\ algorithm instead.
\vspace{-3mm}
\paragraph{MNIST results.}
We consider a simple Jensen-Shannon GAN model trained on the MNIST dataset with latent space dimension $d = 2$. We compare samples obtained by \isir, MALA, and \XTryM\ from the energy-based model associated with $E_{JS}(z)$, see \eqref{eq:energy_funs_GANS}. We use a wide normal distribution as the global proposal for \isir\ and \XTryM, and pools of candidates at each iteration $N = 10$. The step-size of MALA is tuned to keep an acceptance rate $\sim 0.5$. We visualize chains of $100$ steps in the latent space obtained with each method in \Cref{fig:mnist_energy_plots_js}. Note that the poor agreement between the proposal and the landscape makes it difficult for \isir\ to accept from the proposal and for MALA to explore many modes of the latent distribution, as shown in \Cref{fig:mnist_energy_plots_js}. \XTryM\ combines effectively global and local moves, encouraging better diversity associated with a better mixing time. The images corresponding to the sampled latent space locations are displayed in \Cref{fig:mnist_images_visualize} and reflect the diversity issue of MALA and $\isir$. Further details and experiments are provided in \Cref{supp:sec:MNIST}, including similar results for WGAN-GP \cite{gulrajani:2017:wgan} and the associated EBM $E_{W}(z)$.
\vspace{-3mm}

\begin{figure}%[h]
\centering
\begin{subfigure}{0.8\textwidth}
\captionsetup{justification=centering}
\includegraphics[width=1.0\textwidth]{figures/MNIST/energy_landscape_2d_gan_mnist.pdf}
\end{subfigure}
\vspace{-2mm}
\caption{MNIST energy landscape and single chain latent samples visualizations.}
\label{fig:mnist_energy_plots_js}
\vspace{-5mm}
\end{figure}

\paragraph{Cifar-$10$ results.}
% We consider the problem of sampling from the energy-based models, defined by the energy functions $E_{JS}(z)$ and $E_{W}(z)$ from \eqref{eq:energy_funs_GANS}.
We consider two popular architectures trained on Cifar-10, DC-GAN~\cite{radford2016unsupervised} and SN-GAN~\cite{miyato2018spectral}. In both cases the dimension of the latent space equals $d = 128$. Together with the non-trivial geometry of the corresponding energy landscapes, the large dimension makes sampling with NUTS unfeasible in terms of computational time. We perform sampling from mentioned GANs as energy-based models using \isir, MALA, \XTryM, and \FlXTryM. In \isir\ and \XTryM\ we use the prior $p_{0}(z)$ as a global proposal with a pool of $N=10$ candidates. For \FlXTryM\, we perform training and sampling simultaneously. Implementation details are provided in \Cref{supp:sec:cifar}. To evaluate sampling quality, we report the values of the energy function $E(z)$, averaged over $500$ independent runs of each sampler. {We also visualize the inception score (IS) dynamics calculated over $10000$ independent trajectories}. We present the results in \Cref{fig:cifar_10_pictures} together with the images produced by each sampler. Note that \XTryM\ and \FlXTryM\ reach low level of energies faster than other methods, {and reach high IS samples in a limited number of iterations}. Visualizations indicate that MALA is unlikely to escape the mode of the distribution $p(z)$ it started from, while \isir\ and \XTryM/\FlXTryM\ better explores the target support. However, global move appear to become more rare after some number of iterations for \XTryM/\FlXTryM, which then exploit a particular mode with MALA steps. We here hit the following limitation: $\isir$ remains at relatively high-energies, failing to explore well modes basins but still accepting global moves, while \XTryM/\FlXTryM\ explores well modes basins but eventually remains trapped. We predict that improving further the quality of the \FlXTryM\ proposal by scaling the normalizing flow architecture would allow for more global moves.See \Cref{supp:sec:cifar} for additional experiments (including ones with SN-GAN), {FID dynamics}, and visualizations.



\begin{figure}%[h]
\centering
\begin{subfigure}{0.29\textwidth}
\includegraphics[width=1\textwidth]{figures//MNIST/samples_isir_2d_mnist.pdf}
\caption{\isir\ samples}
\label{fig:samples_mnist_2d_ex2mcmc}
\end{subfigure}
\hspace{4mm}
\begin{subfigure}{0.29\textwidth}
\includegraphics[width=1\textwidth]{figures//MNIST/samples_mala_2d_mnist.pdf}
\caption{MALA samples}
\label{fig:samples_mnist_2d_ex2mcmc}
\end{subfigure}
\hspace{4mm}
\begin{subfigure}{0.29\textwidth}
\includegraphics[width=1\textwidth]{figures//MNIST/samples_ex2mcmc_2d_mnist.pdf}
\caption{\XTryM\ samples}
\label{fig:samples_mnist_2d_ex2mcmc}
\end{subfigure}
\caption{MNIST samples visualization. -- Single chains run, sequential steps.}
\label{fig:mnist_images_visualize}
\vspace{-5mm}
\end{figure}

\begin{figure}%[h]
\centering
\begin{subfigure}{0.3\textwidth}
\captionsetup{justification=centering}
\includegraphics[width=1.0\textwidth]{figures/energy_dcgan.png}
\caption{Energy decay for $100$ iterations}
\label{fig:energy_dc_gan_vis}
\end{subfigure}
\begin{subfigure}{0.25\textwidth}
\captionsetup{justification=centering}
\includegraphics[width=1.0\textwidth]{figures/is_dcgan.pdf}
\caption{IS dynamics, $1000$ iterations}
\label{fig:energy_dc_gan_vis}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
\includegraphics[width=1\textwidth]{figures/samples_ex2.png}
\caption{\XTryM\ samples}
\label{fig:samples_cifar_iters}
\end{subfigure}

\begin{subfigure}{0.48\textwidth}
\captionsetup{justification=centering}
\includegraphics[width=1.0\textwidth]{figures/samples_mala.png}
\caption{MALA samples}
\label{fig:mala_cifar_10_vis}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\captionsetup{justification=centering}
\includegraphics[width=1.0\textwidth]{figures/samples_isir.png}
\caption{\isir\ samples}
\label{fig:isir_cifar_10_vis}
\end{subfigure}
\caption{Cifar-$10$ energy and sampling results with DC-GAN architecture. Along the horizonthal lines we visualize each $10$th sample from a single trajectory.}
\label{fig:cifar_10_pictures}
\vspace{-5mm}
\end{figure}


==> sec_related.tex <==
% \isir\ was proposed by~\cite{andrieu2010particle} and further developed in~\citep{andrieu2018uniform}; see also~\citep{lee2010utility,lee2011auxiliary}.

%\isir\ has connections to particle Gibbs methods, as highlighted in \cite{andrieu2018uniform}. The main difference is that the proposal distribution for the latter is defined on the ''path space'' used in sequential Monte Carlo methods; see also~\citep{doucet2015efficient}. Using this analogy, the rejuvenation kernel of \XTryM\ plays a role similar to that of the backward sampling kernel in particle Gibbs with backward sampling (PGBS; \cite{lindsten2013backward}). \marylou {Maybe this should be developed?} \eric{only partially true}

%\XTryM\ algorithm can also be considered as a summarized version of the Gibbs sampler proposed in~\citep{tjelmeland2004using}. \marylou{Is this the case for \isir~ or just \XTryM?}


% Related works focusing on adaptive schemes
\vspace{-3mm}
The possibility to parametrize very flexible probabilistic models with neural networks thanks to deep learning has rekindled interest in adapting MCMC kernels; see \eg\  \cite{song2017nice,Hoffman2019,albergo:2019,Nicoli2020,Hackett2021}. While significant performance gain were found in problems of moderate dimensions, these learning-based methods were found to suffer from increasing dimensions as fitting models accurately becomes more difficult \cite{DelDebbio2021,Mahmoud2022}. Similarly to \FlXTryM, a few work proposed adaptive algorithms that alternates between global and local MCMC moves to ensure ergodicity without requiring a perfect learning of the proposal\cite{Pompe2020,Gabrie2021}. {More precisely}, \cite{Pompe2020} focused on multimodal distributions and analysed a mode jumping algorithm using proposals parametrized as mixture of simple distributions. While \cite{Gabrie2021}, closer to this work, introduced a combination of a local and a global sampler {leveraging normalizing flows} with a more classical choice for the global sampler: independent Metropolis-Hasting (IMH) instead of \isir. {The present work builds on these previous propositions of combinations of local and global sampler by clarifying the reasons of their effectiveness through entirely novel detailed mathematical and empirical analyses. We chose to focus on $\isir$ with an adaptive proposal as the global sampler since (i) the learning component allows to tackle high-dimensional targets, (ii) theoretical guarantees can be obtained for \isir~whereas IMH is more difficult to analyze, (iii) IMH and \isir~(as a multiple-try MCMC) are expected to have similar performances for comparable computational budget \cite{bedard2012scaling} but IMH is sequential where $\isir$ can be parallelized by increasing the number $N$ of proposals per iteration.}


Another line of work exploits both normalizing flows and common local MCMC kernels for sampling \cite{Parno2018,Hoffman2019,Noe2019,Zhang2022}, {yet following the different paradigm of using the flow as a reparametrization map, a method sometimes referred to as neural transport:} the flow $T$ is trained to transport a simple distribution $\proposalbase$ near $\target$, which is equivalent to bringing $\pushforward[T^{-1}][\target]$ (the pushforward of the original target distribution $\target$ by the inverse flow $T^{-1}$) close to $\proposalbase$. If $\proposalbase$ is simple enough to be efficiently sampled by local samplers, the hope is that local samplers can also obtain high-quality samples of $\pushforward[T^{-1}][\target]$ -- samples which can be transported back through $T$ to obtain samples of $\target$. This method {attempts} to reparametrize the space to disentangle problematic geometries for local kernels. Yet, it is unclear what will happen in the tails of the distribution for which the flow is likely poorly learned. Furthermore, in order to derive an ergodicity theory for these transported samplers, \cite{Parno2018} necessitated substantial constraints on maps (see section 2.2.2.).  


